Navigation Method Enhancing Music Listening Experience by Stimulating Both Neck Sides with Modulated Music Vibration

We propose a method that stimulates musical vibration (generated from and synchronized with musical signals), modulated by the direction and distance to the target, on both sides of a user's neck with Hapbeat, a necklace-type haptic device.We conducted three experiments to confirm that the proposed method can achieve both haptic navigation and enhance the music-listening experience.Experiment 1 consisted of conducting a questionnaire survey to examine the effect of stimulating musical vibrations.Experiment 2 evaluated the accuracy (deg) of users' ability to adjust their direction toward a target using the proposed method.Experiment 3 examined the ability of four different navigation methods by performing navigation tasks in a virtual environment.The results of the experiments showed that stimulating musical vibration enhanced the music-listening experience, and that the proposed method is able to provide sufficient information to guide the users: accuracy in identifying directions was about 20 deg, participants reached the target in all navigation tasks, and in about 80% of all trials participants reached the target using the shortest route.Furthermore, the proposed method succeeded in conveying distance information, and Hapbeat can be combined with conventional navigation methods without interfering with music listening.

==> Don't use/README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

IEEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> Don't use/sub0-abst.tex <==
%0概要
\begin{abstract}
% 背景
The vibroacoustic effect plays a vital role in enhancing the experience of entertainment content, but it can be enjoyed only in certain facilities and limited environments.
% 提案
In a previous study, we proposed a vibration mechanism using motors and a thread to output high-power, low-frequency vibration.
In this paper, we propose a practical necklace-type haptic device using the proposed mechanism, named Hapbeat, to promote uses of the vibroacoustic effect.
% 小型軽量について説明する。
The Hapbeat weighs only 58.5 grams, is pressure-free, can be worn within five seconds, and is battery-powered.
% 実験結果
To demonstrate Hapbeat's characteristics, we measured the vibrations transmitted to six subjects using accelerometers at a total of 32 measurement points on the chest, neck-side, and nape areas.
Using 20 Hz, 80 Hz, and 140 Hz sine waves with an amplitude consuming 1 W at Hapbeat's motors as input signals, the Hapbeat transmits vibrations of about 10--50 $\mathbf{m/s^{2}}$ (summation of triaxial root-mean-square values) to a distance of 1 cm from Hapbeat's ribbon.
A frequency response measurement shows the Hapbeat can output more than 10 $\mathbf{m/s^{2}}$ from a 5--270 Hz sine wave input with 1 W consumption, and a response time of 2.74 milliseconds.
% 結論
% おわり
Our proposed method will help the development of usable and high-performance vibroacoustic devices, which are important for promoting uses of the vibroacoustic effect.
\end{abstract}
\begin{IEEEkeywords}
Haptic Display, Entertainment, Human-Computer Interaction.
\end{IEEEkeywords}
\IEEEpeerreviewmaketitle
%1序論
\section{Introduction}
The vibroacoustic effect, which plays a vital role in enhancing the experience of music, movies, and other entertainment content, is mainly due to air pressure changes from the sound source acting on the entire body directly or via a solid intermediary.
This haptic sensation can be felt from sources such as the heavy bass sound from large sub-woofers installed in live-music venues, clubs, and cinemas, the explosion of fireworks, and the sounds of guns and bombs during military maneuvers.
The sensation is difficult to create in daily life owing to the cost of equipment and the requirement for loud noises. Although recent technological developments enable the enjoyment of entertainment events remotely, many people still opt to attend in person \cite{liveMusicRevenue}.
To overcome these challenges, researchers are developing a way to generate vibroacoustic sensations using haptic devices with vibrators, contributing to the enhancement of the immersive experience of entertainment content \cite{karam2010emoti}, \cite{konishi2016synesthesia}, \cite{subpac}, \cite{woojer}, \cite{bhaptics}.
\par
However, many small vibrators or a few large vibrators need to be embedded in the devices to achieve a wide range of vibration transmissions. Consequently, such devices become large, expensive, and uncomfortable to use.
The mechanism of using an eccentric motor and linear vibrators, including the general speaker, commonly used in general haptic devices is what causes the size and expense (Fig. \ref{fig:desc_vibration_mechanism} (a)).
All these general vibrators use the reaction force by moving the internal weight.
To increase the output in the ultra-low frequency band (below 20 Hz), which is an essential band for vibroacoustic effects, the mass and stroke of the internal weight, in terms of momentum, need to increase.
This mechanical requirement causes the challenging trade-off between the device size and high-power, low-frequency vibrational output.
\par
The high-frequency band in the tactile domain (100--1000 Hz), which is the sensitive band of the skin’s Pacinian corpuscles \cite{sato1961response}, also cannot be underestimated.
The experiment undertaken by Merchel et al. \cite{merchel2013music} revealed that vibrations of high frequency from speakers on the stage at a concert hall reached the audience seats.
The response time is also important.
Previous studies on the synchronization of auditory and tactile stimuli have shown that asynchrony can be distinguished in about 20--50 milliseconds \cite{adelstein2003sensitivity}, \cite{balandra2019sensitivity}, \cite{levitin2000perception}, so the delay in the vibrators should be less than this value.
\par
Our previous study proposed a vibration generation mechanism using motors and a thread (Fig. \ref{fig:desc_vibration_mechanism}(b)) that solves the trade-off \cite{yamazaki2016tension}.
We developed and evaluated a body-wound prototype called the Wearable Tension-based Vibroacoustic Device (hereafter referred to as WTV) shown in Fig. \ref{fig:desc_vibration_mechanism}(c).
The study demonstrated that a small device can in principle transmit powerful low-frequency vibrations over a wide area. However, the WTV has several problems in practical usage: it is troublesome and uncomfortable to wear, and the actuators consume large amounts of electricity which generate significant heat and increase the size of driver circuits.
\par
This study aims to demonstrate a practical wearable device using our mechanism that can transmit low-frequency vibration over a wide area of the user's body.
We developed a necklace-type device called the Hapbeat\footnote{
We originally named Hapbeat for any haptic device using one or more motors and threads, so Hapbeat can form not only a necklace-type. However, we define Hapbeat as a necklace-type device in this paper for clarification.
}
and tested (1) the performance of vibration transmission on the user's body, and (2) the fidelity of vibration waveform compared to input signals.
We also list key elements to be considered in downsizing, and tested the effect of altering the device form from body-wound type (the WTV) to a necklace-type (the Hapbeat).
% figure
\begin{figure}[hbt]
\begin{center}
\includegraphics[width = 8cm]{figures/desc_vibration_mechanism.png}
\end{center}
\caption{
The mechanism of (a) linear vibrators and (b) the proposed mechanism. The red arrows indicate actuator movement, and the blue arrows indicate movement driven by the actuator. The blue and green dots in the top and sectional views in (b) correspond to each other and indicate the maximum and minimum states of the output for a sinusoidal wave input. Here $r$ stands for the distance between the thread to be reeled out and the center of the bobbin, which can be approximated to the inner radius of the bobbin. (c) The body-wound prototype proposed in our previous study.
}
\label{fig:desc_vibration_mechanism}
\end{figure}
%2関連研究
\section{Related Works}
Much research has been carried out on the transmission of vibrations to a wide area of the human body to enhance the experience of entertainment content.
\par
% 小型振動子デバイスの説明
For example, previous studies proposed clothing-type and chair-type haptic devices embedded with several small vibrators to directly stimulate any part of the body \cite{konishi2016synesthesia}, \cite{lemmens2009body},  \cite{chandra2020preliminary}, \cite{israr2012surround}, \cite{5196671}.
Due to their high spatial resolution, these haptic devices are suitable for conveying complex information such as distance or direction by stimulating arbitrary areas.
However, small vibrators cannot sufficiently output low-frequency vibrations, and incorporating more vibrators increases manufacturing costs and breaking risks.
\par
% 大型振動子デバイスの説明
In addition, there are other haptic devices that have only a few large vibrators embedded in the back of a chair or a backpack \cite{karam2010emoti}, \cite{subpac}, \cite{woojer}, \cite{nanayakkara2009enhanced}.
These devices have a low spatial resolution, but their large contact area contributes to the transmission of vibrations over a wide area of the user’s body.
They can also generate stronger low-frequency vibrations compared to small vibrators because the mass and stroke of the internal weight are larger.
This type of haptic device is thus suitable for displaying the vibroacoustic effect, typically encountered when watching movies or listening to music.
However, portability is not an option owing to the device size.
Consequently, the chair-type device has restrictions on location and posture, and the backpack-type device has limitations due to the load, such as weight and tightness.
Heavy internal weight also sacrifices response time and high-frequency output, and extra components such as the chair or backpack increase the overall cost.
\par
% 工夫した例の説明
Some studies have proposed different approaches to efficiently transfer vibrations over a wider area.
Sakuragi et al. \cite{sakuragi2015collarbeat} used bone conduction and showed that a clavicle can effectively be attached to a vibrator.
Kurihara et al. \cite{kurihara2014large} incorporated particles of granular Styrofoam as a medium to convey vibration from an audio speaker to the contact area.
Withana et al. \cite{withana2015rippletouch} applied properties of low-frequency acoustic wave propagation in the human body and proposed a low-resolution haptic interface that is capable of providing haptic stimulation to multiple areas of the body via a single point-of-contact actuator.
These approaches involve vibration transmission through an object, which allows for a larger transmission area with fewer vibrators and a simpler device compared to the devices mentioned earlier.
However, the vibrators in these applications are conventional and do not, therefore, resolve the aforementioned trade-off.
\par
% モーターをアクチュエータとして利用した例
In contrast, Yem et al. \cite{yem2016vibrotactile} show that DC motors are effective vibrators capable of driving low-frequency vibrations by harnessing the rotational motor’s counter force and using the rotor of the motor as the vibration mass.
In addition, Minamizawa et al. \cite{minamizawa2007gravity} and Nakamura et al. \cite{nakamura2017hapbelt} used a belt in contact with a fingertip and a rotational motor as a driver.
The deformed skin artificially generated sensations such as holding an object or the feeling of collision and traction in a video game.
The rotational motion of the motor shaft, as the source of vibration, is ultimately converted into a translational motion of the skin.
The skin displacement can be increased, and static forces and low-frequency vibrations can be effectively represented.
However, these studies focus on the fingertips, i.e., a localized area, and differ from the purpose of this paper, which is to transmit vibrations over a wide area.
%3提案手法
\section{Proposal}
We propose a compact necklace-type haptic device that can transmit high-power, low-frequency vibrations to a wider area of the user’s body using our proposed mechanism (Fig. \ref{fig:desc_vibration_mechanism}(b)).
\par
% 課題の解決説明
As described in related works, the challenges facing current haptic devices are their heaviness, large size, and inability to produce high-power, low-frequency vibration output over a wide area.
This is due to the use of eccentric motors or linear vibrators.
Our previous work \cite{yamazaki2016tension} demonstrated that our proposed mechanism extensively transmits high-power, low-frequency vibrations independent of the device size, and thus can solve the challenges.
\par
Here, we explain the proposed mechanism (Fig. \ref{fig:desc_vibration_mechanism}(b)) and prototype (Fig. \ref{fig:desc_vibration_mechanism}(c)) from our previous study.
The bobbin is attached to the shaft, and the thread is tied to the bobbin.
The thread contacts the user's body and drives the skin, acting as a transmission mechanism.
The other end of the thread is wound around the bobbin several times and then rolled out of the enclosure.
The thread is wound around the user’s body and then similarly wound and fixed to another bobbin attached to a motor shaft located on the opposite side.
Thus, the rotational movement of the shaft is converted into a translational movement of the thread.
The area of the body in contact with the thread is actuated, thereby transmitting vibration.
The thread is wound onto the bobbin, and thus the maximum stroke amplitude is determined by the bobbin capacity and the thread volume.
The volume is relatively small compared to the capacity of the bobbin, making it possible to generate high-power, low-frequency vibrations in a small enclosure.
The thread, a transmission mechanism, contacts extensively to the user's body and thus transmits vibrations over a wide area without increasing the number of actuators.
\par
% ベルト型からネックレス型に変更した理由
We used this mechanism to develop a belt-type device to improve the music listening experience and demonstrated it at an exhibition.
However, the attendees noted the following problems relating to convenience.
First, each time after putting the belt-type device on the body, the tightness needs to be adjusted by altering the length of the belt, a tedious task that takes more than ten seconds.
Second, the transmitted vibration gets weaker when worn over thick clothing, and in some cases users needed to take off or roll up their clothes.
Third, the tightness on the body causes a sense of pressure, which makes it unsuitable for extended use.
\par
By contrast, a necklace-type device does not require adjustment of the ribbon length, and users only have to suspend it from the neck.
Suspending the device puts little pressure on the users, and the device rarely interferes with users' movement.
This makes a necklace-type device suitable for extended use in daily life.
%4実装
\section{Implementation}
\label{implementation}
The structure and components of the Hapbeat are shown in Fig. \ref{fig:desc_hapbeat_mechanism}.
% figure
\begin{figure}[hbt]
\begin{center}
\includegraphics[width=8cm]{figures/desc_hapbeat_mechanism.png}
\end{center}
\caption{
The structure and components of Hapbeat.
(a) The value of $\rho$ indicates the curvature radius of the tube.
(b) The green arrows indicate the direction of the tension applied to the bobbin when the thread is reeled out.
(c) The dimensions of the bobbin, with $\phi$ indicating the diameter of the corresponding part.
}
\label{fig:desc_hapbeat_mechanism}
\end{figure}
The volume is roughly 38 $\mathrm{cm^3}$, the mass is 58.5 grams, and the maximum thread feed length, which corresponds to the full stroke length, is approximately 50 mm.
\par
The enclosure and bobbin were formed by an industrial 3D-printer (HP Development Company LP, HP Jet Fusion 4200, PA12).
For implementation, a rigid thread, coreless motor, and steady torque are required.
Although a belt could transmit the vibrations, as used in related works \cite{minamizawa2007gravity}, \cite{nakamura2017hapbelt}, we adopted a polyethylene line as the thread component (RUNCL PowerBraid, four strands, strength/diameter is 52.2 kg/0.50 mm, gray).
It is rigid and thus effectively reflects the shaft's movement; it is easy to store inside the bobbin, contributing to downsizing and weight reduction.
Additionally, a satin ribbon (6 mm wide, 100\% polyester) is used for contact components to the user's body.
The ribbon is connected to the thread by plastic couplings.
\par
The motor should be coreless with a low moment of inertia to allow quick repetitions of forward and reverse rotation.
The coreless motor used in Hapbeat was ordered with the following characteristics: 3 V rated voltage, 1.1 $\Omega$ armature resistance, 1.92 W maximum output, 6.8$\mathrm{\times10^{-3}  N\cdot m}$ stall torque, 10 milliseconds mechanical time constant, 0.6 $\mathrm{G \cdot cm^2}$ rotor moment of inertia, and 110$\mathrm{\times10^3 rad/s^2}$ angular acceleration.
\par
% 定常張力の説明
\subsection{Implementation of steady-state torque}
To properly convert a signal applied to the motor into translational motion, the thread must be sufficiently wound on the bobbin while suspended from the user’s neck.
For this reason, generating a steady-state torque is necessary to prevent the thread from unrolling off the bobbin.
Applying an offset voltage to the motor is desirable in terms of simplicity and waveform fidelity, but not practical because of the increase in power consumption, heat generation, and deterioration of the motor.
\par
Instead, a rubber cord (KawamuraSeichu Co Ltd, elastic cord, 1 mm diameter, white, made of natural rubber and rayon, 36 mm length) was used as a spring material, which combines thinness and high elongation rate.
One end of the rubber cord was fixed to the bobbin (Fig. \ref{fig:desc_hapbeat_mechanism}(a) yellow circle part) and the other end to the enclosure (Fig. \ref{fig:desc_hapbeat_mechanism}(a) green circle part), applying counter-torque when the thread is unrolled from the bobbin (see the green arrows in Fig. \ref{fig:desc_hapbeat_mechanism}.)
For this purpose, the bobbin has three flanges (Fig. \ref{fig:desc_hapbeat_mechanism}(c)).
\par
\subsection{Incorporation into the housing}
\label{Incorporate}
For practical use, exposing the motor should be avoided due to the risk of burns from its heat generation, and thus the motor is incorporated in the housing.
Minimizing the friction of the thread and rubber cord should be considered to maintain the efficiency of vibration transmission, and they are guided by
Teflon tubes (Chukoh Chemical Industries Ltd, PTFE tube, inner diameter $\times$ outer diameter is 1 mm $\times$ 3 mm for the string and 1.5 mm $\times$ 2.5 mm for the rubber cord).
The Teflon tubes were bent to minimize the housing, as shown in Fig. \ref{fig:desc_hapbeat_mechanism}, with their curvatures as large as possible to reduce friction.
A general mini-stereo audio cable was used for compatibility to connect the motor and a drive circuit, and a mini-stereo jack was soldered to the motor terminals.
\par
\subsection{Circuit design}
\label{imp:circitDesign}
To enable Hapbeat to be used everywhere, the drive circuit should be battery powered and ideally be recharged with a general 5 W output USB charger.
A commercial audio amplifier can drive Hapbeat by audio signals.
However, Hapbeat requires a relatively high current of more than 1 A, meaning a 20 W output class amplifier is required, which is inconvenient.
\par
Thus, we designed a drive circuit for Hapbeat which can draw a high current with audio signals and a battery.
FETs (Toshiba Electronic Devices \& Storage Corporation, TPC8408) connected to the output of class-D amplifier ICs (Diodes Incorporated, PAM8403) reduce the output impedance.
Additionally, general audio amplifiers cut off frequencies below 20 Hz to improve sound quality, which is unsuitable for Hapbeat.
To lower the cut-off frequency, we adjusted parameters of resistors and capacitors, which form a high-pass filter at the input of the amplifier IC: the resistors were set at 10 $\mathrm{k\Omega}$ and the capacitors to 2.2 $\mathrm{\mu F}$, resulting in a cut-off frequency of 7.2 Hz.
% 回路図は無くても良いのでは？指摘されたら足す。
% 該当部分の回路図を図\ref{fig:desc_schema}に示す。
\begin{figure}[hbt]
\begin{center}
\includegraphics[width = 7cm]{figures/desc_schema.png}
\end{center}
\caption{
Schematic of the drive circuit focused on output part.
}
\label{fig:desc_schema}
\end{figure}
\subsection* {Evaluation of the drive circuit}
\label{exp:evaluateCircuit}
We compared the performance of the drive circuit and a commercial audio amplifier (Lepy, LP-V3S, 25 W output; hereafter referred to as Lepy) in terms of frequency response and total harmonic distortion (THD).
Input signals were sine waves of 0.5 V amplitude at frequencies based on the E12 series values (1.0, 1.2, 1.5, 1.8, 2.2, 2.7, 3.3, 3.9, 4.7, 5.6, 6.8, 8.2; these values times 1, 10, 100 for a total of 36 values in 1--820 Hz, and 1000 Hz).
A function generator (FeelTech, FY6600-30) was used to input the signals to the drive circuit and Lepy.
An oscilloscope (Tektronix Inc, MDO4024C) recorded the output signals from the designed circuit and Lepy with a sampling rate of 1 kHz for 1--8.2 Hz input and 10 kHz for input over 10 Hz.
The measurement was conducted three times with the maximum volume of the designed circuit and Lepy.
The THD values were calculated using the thd functions of MATLAB (The MathWorks Inc, version R2021b) with the harmonic number of six.
The derivation equation is as follows.
\begin{equation*}
THD=\frac{\sqrt{V_{1}^{2} +V_{2}^{2} +V_{3}^{2} +V_{4}^{2} +V_{5}^{2} +V_{6}^{2}}}{V_{0}}
\end{equation*}
where $V_0$ is the RMS value of the fundamental component and $V_1$--$V_6$ are the RMS values of the $n$th harmonic voltage.
\begin{figure}[hbt]
\begin{center}
\includegraphics[width = 8cm]{figures/result_amp_comparison.png}
\end{center}
\caption{
Frequency response result of the designed circuit and Lepy.
The maximum standard deviation of the gain is 0.011 dB for both amplifiers, and that of the THD is 0.72 dB for the Hapbeat and 1.22 dB for Lepy.
}
\label{fig:result_amp_comparison}
\end{figure}
\subsubsection*{\textbf{Result \& Discussion}}
The result is shown in Fig. \ref{fig:result_amp_comparison}.
Although the drive circuit is battery-powered, it showed better performance than Lepy for 1--22 Hz input.
This indicates that the circuit is more suitable for driving Hapbeat, which must be good at driving input signals below 20 Hz.
%5評価
\section{Evaluation}
In the experiment 1, we measured the transmitted vibration on subjects to verify the Hapbeat can transmit low-frequency vibration over a wide area.
In the experiment 2, we investigate the power consumption, starting current, effect of the Hapbeat enclosure mass, and the response time to inputs to evaluate the effect of altering the device form from body-wound type (WTV) to necklace type (Hapbeat).
\par
% 身体への振動伝達、複数回実施。目的1：Hapbeatの低周波振動が広範囲に伝わっていることを確認。被験者実験を行う際にどの測定点で測定するのが妥当かを検証
\subsection*{Experiment 1: Vibration transmission to the subject’s body}
\subsection{Detailed examination of vibration transmission}
\label{exp:repeat_exp}
In this experiment, transmitted vibrations were measured at 71 locations on one subject (30-year-old male, 174 cm height, 74 kg weight, and 24.3\% body fat) to determine the necessary and sufficient measurement locations for evaluating transmissions.
The measurement locations were placed as shown in Fig. \ref{fig:desc_position}, dividing the area into three sections: the chest, neck-side, and nape.
Hereafter, the measurement points are written as numbers with a hash, e.g., \#7 shows measurement point 7 in Fig. \ref{fig:desc_position}.
\begin{figure}[hbt]
\begin{center}
\includegraphics[width = 8cm]{figures/desc_position_v2.png}
\end{center}
\caption{
Location of measurement points.
The blue numbers are identification numbers of measurement points in each area.
The magenta framed identification numbers indicate the measurement points on the clavicle or stitch.
The black numbers show the length in centimeters, and the blue numbers identify the points.
The green measurement points are extracted points used in section \ref{exp:subject_exp}.
The red circled letters are reference points in each row, determined by the following criteria: (A) contact point between the ribbon and the clavicle; (B) middle point between (A) and (C); (C) center of the coupling; (D) the middle point of the housing; (E) cross point between the ribbon and the stitch extension line; and (F) center of the cervical vertebrae (approximate).
}
\label{fig:desc_position}
\end{figure}
The input sine wave voltages from the function generator were adjusted to consume 0.5 W, 1 W, and 2 W at 20 Hz, and 1 W at 80 Hz and 140 Hz by one motor.
Hereafter, the signal types are expressed as [frequency]-[power consumption], e.g., 20Hz-1W shows the input signal with a frequency of 20 Hz and a voltage adjusted to consume 1 W by one motor.
The transmitted vibration from the Hapbeat was measured with an analog triaxial accelerometer (NXP Semiconductors, MMA7361LC, using 6 G mode).
\par
Assuming a casual scene as a use case of Hapbeat, the subject wore a T-shirt or dress shirt and underwear.
The clothes worn are all are made by Uniqlo Co., with the T-shirt being a U Crew Neck short-sleeved T-shirt, the dress shirt a men’s 100\% extra-fine cotton broadcloth long-sleeved shirt, and underwear an AIRism Micro Mesh V-neck short-sleeved singlet 83\% nylon and 17\% spandex.
The friction coefficients and Young's moduli of the T-shirt and dress shirt are shown in Table \ref{tab:clothing}.
\par
\begin{table}[]
\centering
\caption{Friction coefficient and Young's modulus of the clothing}
\label{tab:clothing}
\scalebox{1}
{
\begin{tabular}{rl|cc}
Clothing    & Direction  & \begin{tabular}{c} Friction \\ Coefficient \end{tabular}
& \begin{tabular}{c} Young's \\ modulus \end{tabular} \\ \hline
T-shirt     & Vertical   & 0.188                & 573 $N/mm^2$    \\
& Horizontal & 0.203                & 546 $N/mm^2$ \\
Dress shirt & Vertical   & 0.179                & 17.6 $N/mm^2$ \\
& Horizontal & 0.178                & 11.0 $N/mm^2$
\end{tabular}
}
\end{table}
\par
The friction coefficients were measured by a surface tester (Kato Tech Co Ltd, KES-FB4-A).
A 20 cm $\times$ 20 cm sample was prepared and tested six times using a weight of 400 grams (for applying tension on the sample), and the average value calculated.
Young's moduli were measured by a tensile tester (A\&D Co Ltd, RTF-1250), with the test performed according to the Tensile Test of Fabrics (JIS L 1096 Strip Method).
%
Five samples were cut from the vertical and horizontal directions of the T-shirt, and three from the dress shirt.
Each sample dimension was 50 mm $\times$ 300 mm, and the gauge length during the test was 200 mm.
Tests were conducted on each sample, and the average values were then calculated.
\par
For comparison with Hapbeat, we used a Vp2 (Acouve Laboratory Inc, Vp210) as a representative of linear vibrators.
The transmitted vibrations from the Vp2 were measured at the points on the red line in Fig. \ref{fig:desc_position}.
Signals of 20Hz-2W, 80Hz-2W, and 140Hz-2W were inputted to the Vp2.
The Lepy was used to drive the Vp2 because the driver circuit of the Hapbeat cannot drive Vp2 sufficiently due to the Vp2's high resistance (10 $\mathrm{\Omega \pm15\%}$, which is about ten times larger than that of the Hapbeat motor).
The input signal voltage was set to consume 2 W by the Vp2 to match the total power consumption of the Hapbeat, which consists of two motors.
A rubber belt (Kiyohara \& Co Ltd, SUN40-163, made of Lycra, elongation is 120\%, 25 cm width) with a buckle attached the Vp2 on the subject.
The length of the rubber belt, including the buckle, was determined as follows.
The Vp2 was temporarily attached to the subject using double-sided tape (Aderans Co Ltd, AD\&F Wig double-sided hard tape) at the same location as the Hapbeat in Fig. \ref{fig:desc_position}.
The circumference of the subject's body, including the attached Vp2 height, was then measured, with 75\% of the measured circumference becoming the rubber belt length.
\subsubsection*{\textbf{Procedure}}
Initially, the measurement points were marked on the subject’s body with a pen, as well as an outline of the enclosure, so that it could be restored to the initial location if the Hapbeat was misaligned during the experiment.
The accelerometer was then attached to the measurement point with its x-axis parallel to the green and yellow arrows in Fig. \ref{fig:desc_position}, and z-axis perpendicular to the body surface.
To maintain the attachment, an experimenter held the accelerometer cable 20 cm from the sensor part.
At each measurement point, measurements were made once for input signals of 20Hz-0.5W, 20Hz-1W, 20Hz-2W, 80Hz-1W, and 140Hz-1W.
The subject stabilized his posture during the experiment by following these instructions: sit on a chair with your upper body perpendicular to the seat surface, lightly press your back and head against the pole fixed directly behind the chair, and keep your eyes at the same level throughout the experiment (level with an object in the room).
These procedures was conducted three times for the T-shirt and dress shirt.
\par
\subsubsection*{\textbf{Result \& Discussion}}
The results are shown in Fig. \ref{fig:result_trans_repeat}.
Hereafter, we evaluate the magnitude of the transmitted vibration by root-mean-square values of measured accelerations designated as $ACC_{RMS}$ derived from eq. (\ref{eq:value}):
\begin{equation}
ACC_{RMS}\ =\ RMS_{x} +RMS_{y} +RMS_{z}, \label{eq:value}
\end{equation}
\begin{equation}
RMS_{x} =\sqrt{\frac{1}{N}\sum\limits _{n=1}^{N} |x_{n} -\mu |^{2}},
\;\;\; \mu \ =\ \frac{1}{N}\sum _{n=1}^{N} x_{n},   \label{eq:rms}
\end{equation}
where $x_{n}$ is sampled data, $N$ = 10 k (points), and eq. (\ref{eq:rms}) has equivalent y-axis and z-axis forms.
Selected measurement points used in the experiment in section \ref{exp:subject_exp} are shown as green points in Fig. \ref{fig:desc_position}.
The reasons for the selection are described below.
\par
For the chest and neck-side areas, we only selected points located on the right side because $ACC_{RMS}$ and the attenuation tendency of both sides seemed similar. Investigating the asymmetry is beyond our purpose.
For the neck-side and nape areas, we first selected all points located near the ribbon because the large $ACC_{RMS}$ indicated importance for perception.
Then we selected center points located far from the ribbon because the $ACC_{RMS}$ of the skin points at the same distance from the ribbon (e.g., \#2, \#7, and \#12 in the neck-side area) differed within only $\pm 0.071 \mathrm{m/s^{2}}$ at most.
Additionally, the large-small relationships among the points seemed similar to those of near-ribbon points.
\par
For the near-ribbon points in the chest area, we selected \#11, \#12, and \#13 rather than \#15, \#16, and \#17.
The trends were similar, and we wanted to observe the vibration damping.
For the rest of the points, we selected them to observe vibration damping. 
The clavicles (\#1, \#6, and  \#10) may reflect the effect of body shape. The damping trends from the housing (\#5, \#10, and \#14) and the clavicle or coupling contact ((A) and (C) in Fig. \ref{fig:desc_position}) may differ from other points.
\begin{figure*}[hbt]
\begin{center}
\includegraphics[width = 17cm]{figures/result_trans_repeat.png}
\end{center}
\caption{
Results of vibration transmission conducted on the subject, who is sub-6 shown in Table \ref{tab:subject_info}.
The size of the circles indicates the magnitude of $ACC_{RMS}$ and the colors indicate input signal type.
}
\label{fig:result_trans_repeat}
\end{figure*}
\par
The result of Vp2 shown in Fig. \ref{fig:result_Vp2_repeat} demonstrates that the Vp2 transmits larger $ACC_{RMS}$ than the Hapbeat at 80 Hz and 140 Hz, but almost no vibration at 20 Hz.
\begin{figure}[hbt]
\begin{center}
\includegraphics[width = 8cm]{figures/result_Vp2_repeat.png}
\end{center}
\caption{
Results of the acceleration measurement wearing the Vp2.
}
\label{fig:result_Vp2_repeat}
\end{figure}
\par
% 複数の被験者での振動伝達実験。目的：色々な体格の装着者でも、実験\ref{sec:repeat_exp}と同傾向の結果（振動伝達範囲、服による傾向）が得られるかを確認する。
\subsection{Vibration transmission on various body shapes}
\label{exp:subject_exp}
We conducted vibration propagation experiments with six subjects of different body shapes to verify that Hapbeat can extensively transmit powerful low-frequency vibrations, even among users with various body shapes.
The subjects' height, weight, and body fat percentage values measured with a body composition meter (Tanita Corporation, innerScan Dual RD-802) are listed in Table \ref{tab:subject_info}.
The subjects were named sub-1 to sub-6 in ascending order of body fat percentage.
\par
% 被験者の情報テーブル
\begin{table}[hbt]
\centering
\caption{
Information on subjects
}
\label{tab:subject_info}
\scalebox{1}
{
\begin{tabular}{r|cccccc}
& sub-1 & sub-2 & sub-3& sub-4 &sub-5 & sub-6 \\ \hline
Height (cm)              & 185  & 160  & 164  & 165  & 178  & 174  \\
Weight (kg)              & 61.8 & 47.3 & 52.4 & 56.8 & 61.1 & 74.1 \\
Body-fat (\%) & 12.1 & 12.3 & 16.9 & 18.7 & 18.8 & 24.3
\end{tabular}
}
\end{table}
\par
The experimental procedure was the same as in section \ref{exp:repeat_exp}.
However, to shorten the experimental time, the measurement points were limited to the green points in Fig. \ref{fig:desc_position} for the reasons described in section \ref{exp:repeat_exp}.
One measurement was taken per subject.
\par
We also evaluated the subjective vibration perception for each input signal.
The subjects colored measurement points in a figure---Fig. \ref{fig:desc_position} with all explanatory numbers and letters omitted and all points colored black---with the following criteria: (1) red color where subjects clearly felt the vibration, and (2) blue color where subjects subtly felt the vibration.
The difference between clear and subtle is whether the subjects need to concentrate to perceive the vibration.
Initially, the experimenter touched the measurement points on the subjects’ bodies to make them recognize the locations.
During the experiment, the Hapbeat continuously vibrated the subjects.
No time limit was set for the evaluation, but the subjects were asked not to touch their bodies.
\par
\subsubsection*{\textbf{Result \& Discussion}}
\begin{figure*}[hbt]
\begin{center}
\includegraphics[width = 18cm]{figures/result_trans_subject.png}
\end{center}
\caption{
Result of the vibration transmission measurements conducted on the six subjects.
The six columns of squares located above the bars indicate the result of the subjective experiment.
Fully filled squares indicate the subject clearly felt the vibration, while half-filled squares indicate the subject subtly felt the vibration.
The red-colored numbers indicate the point 1 cm away from the ribbon or housing, and the underlined numbers indicate the points measured on the skin.
}
\label{fig:result_trans_subject}
\end{figure*}
The resulting vibration transmission is shown in Fig. \ref{fig:result_trans_subject} and demonstrates that the Hapbeat transmitted powerful 20 Hz vibrations, $ACC_{RMS}$ of 10 $\mathrm{m/s^{2}}$ or greater, to the subjects' skin and clothing across the chest, neck-sides, and nape areas.
\par
% TシャツとYシャツの比較
Comparing the results of the T-shirts and dress shirts, overall $ACC_{RMS}$ of the dress shirts was greater than that of T-shirts.
This is seemingly due to the larger Young’s modulus of the dress shirt.
% 被験者ごとによって大きく異なる
The $ACC_{RMS}$ on some measurement points differed greatly depending on the subjects.
This is seemingly due to the difference in wearing conditions and subjects' body shape.
\par
%% 主観実験について
% 前面、筐体・結合部付近で知覚が強い。
The subjective result in the dress shirt chest area shows that more than five subjects clearly felt the vibration at \#14, \#21, and \#13, near the hosing or coupling.
The hard contact part probably highlighted the vibration perception.
\par
%%%% 皮膚上での出力と周波数比較
\subsubsection*{\textbf{Vibration propagation on the skin}}
To analyze the vibration transmission on the skin in detail, we extracted measurement points on the skin from the results of the T-shirt neck-side area and arranged by power and frequency as shown in Fig. \ref{fig:result_ampfreq_comparison}.
\begin{figure}[h]
\begin{center}
\includegraphics[width = 8cm]{figures/result_ampfreq_comparison.png}
\end{center}
\caption{
Result of the vibration transmission measurements conducted on the six subjects' skin in the neck-side area.
}
\label{fig:result_ampfreq_comparison}
\end{figure}
Table \ref{tab:dampingRate} lists the damping percentage, calculated from $ACC_{RMS}$ of \#7 divided by that of \#8 times one hundred.
\begin{table}[]
\centering
\caption{
Damping percentage between \#7 and \#8
}
\label{tab:dampingRate}
\scalebox{0.95}
{
\begin{tabular}{r|ccccccc}
Signal type & sub-1 & sub-2 & sub-3 & sub-4 & sub-5 & sub-6 & AVG. \\ \hline
20Hz-0.5W & 38.0 & 44.9 & 73.1 & 29.6 & 42.6 & 50.2 & 46.4 \\
20Hz-1W & 38.1 & 37.4 & 51.1 & 31.8 & 37.9 & 48.7 & 40.8 \\
20Hz-2W & 38.0 & 36.4 & 42.5 & 32.1 & 36.0 & 45.7 & 38.5 \\
\hline
20Hz-1W & 38.1 & 37.4 & 51.1 & 31.8 & 37.9 & 48.7 & 40.8  \\
80Hz-1W & 49.2 & 30.5 & 25.5 & 26.2 & 16.8 & 11.0 & 26.5 \\
140Hz-1W & 17.5 & 21.8 & 12.0 & 14.6 & 8.4  & 7.3  & 13.6
\end{tabular}
}
\end{table}
\par
%% 定量
% 出力が大きくなっても遠方点ではあまり大きくならない?
For the comparison of the output (Fig. \ref{fig:result_ampfreq_comparison}, left column), the transmitted vibration increased for all subjects as the output increased.
The damping tended to be intense as the output increased except for sub-1 and sub-4.
For the comparison of the frequency (Fig. \ref{fig:result_ampfreq_comparison}, right column), the overall transmitted vibration decreased as the frequency increased.
The damping tended to be intense as the frequency increased for all subjects.
\par
%% 主観
%出力比較では目立った差はなかったが、周波数比較では明確に高周波数ほど感じにくくなっていた。
The subjective results show little difference between outputs, whereas the perceived intensity decreased as the frequency increased.
Notably, at \#3 and \#13, only one subject clearly felt the 80 Hz vibration, whereas four subjects clearly felt the 20 Hz vibration, which has a similar $ACC_{RMS}$ to that of 80Hz-1W.
Additionally, most subjects could feel no sensation of 80 Hz and 140 Hz vibrations at the distant points (\#6 and \#7).
\par
% FFTした結果
\subsubsection*{\textbf{Fourier transform}}
To verify the fidelity of the transmitted vibration to the skin, we obtained the frequency component from the data via Fast Fourier Transform (FFT).
The data of three axes were converted to one axis by principal component analysis.
\par
The waveform and FFT results of 20Hz-1W at \#8 in the neck-side area and \#6 in the nape area are shown in Fig. \ref{fig:result_fft}.
As representatives, we selected data that included a high percentage of high frequency (sub-2 for the neck-side and sub-1 for the nape) and 20 Hz (sub-6 for both areas).
\par
\begin{figure}[hbt]
\begin{center}
\includegraphics[width = 8cm]{figures/fft_result.png}
\end{center}
\caption{
Waveform of principal axis and result of Fourier transform.
The top graph in each quarter shows principal axis of acceleration signal from 20 Hz sine wave input.
The bottom graph shows the result of single-sided amplitude spectrum of acceleration signal.
}
\label{fig:result_fft}
\end{figure}
\par
The vibration transmitted to the subjects with relatively high body-fat percentage (e.g., sub-6) tended to consist mainly of 20 Hz vibrations, while for relatively low body-fat percentages (e.g., sub-1 and sub-2) it tended to consist mainly of harmonic vibrations.
The difference in frequency composition of the transmitted vibration on the skin implies that the vibration perception probably differs depending on the subject's body shape, body composition, or worn condition.
%% マネキンで再現可能な周波数応答の測定。目的：20Hz未満の低周波を含む、広範囲の周波数応答を再現可能な手法で測定する。
\subsection{Frequency response of the Hapbeat including below 20 Hz}
\label{exp:freqResponse}
To determine whether the Hapbeat can output low-frequency vibrations below 20 Hz, we measured the frequency response of the Hapbeat with a reproducible method.
A mannequin, made from a public 3D model and by a 3D-printer, was used as a reproducible wearer (Fig. \ref{fig:desc_mannequin}).
A commercial gel sheet was used as a substitute for human skin.
The details are as follows.
Mannequin 3D data is haf020.obj from AIST/HQL Human Body Size and Shape Database 2003 \cite{AIST/HQL2003}.
The model was divided into sections as shown in Fig. \ref{fig:desc_mannequin}(a) and (b), and each section was 3D-printed (using Z-PLA Pro material, laminate thickness of 0.29 mm and infill 10\% hexagonal). The printed parts were attached with double-sided tape.
The gel sheet (Exseal Co Ltd, H0-3K, 3 mm thickness, and Asker C0 hardness) is sticky on one side, and the other is smooth, covered with a urethane film.
The sheet was cut into a 50 $\times$ 500 mm piece and attached around the neck part of the mannequin, and into a 230 $\times$ 290 mm piece which was attached to the chest part.
\par
The experimental environment is shown in Fig. \ref{fig:desc_mannequin}(c)--(e).
Measurements were taken at four locations: on the housing, front (Fig. \ref{fig:desc_mannequin} (c)), side (Fig. \ref{fig:desc_mannequin} (d)), and back (Fig. \ref{fig:desc_mannequin} (e)).
The accelerometer was directly applied on the Hapbeat housing or ribbon by double-sided tape.
The same measurement was also performed with the Vp2 to compare the frequency response of the linear vibrator to that of Hapbeat.
The Vp2 was attached to the gel sheet fixed on a flat aluminum plate, and the accelerometer was directly applied on the Vp2.
For the input signal, we used 1--270 Hz sine waves, considering the maximum bandwidth response of the accelerometer (300 Hz), based on the E12 series described in section \ref{exp:evaluateCircuit}.
The input amplitude of each frequency was adjusted to consume 1 W with the Hapbeat and 2 W with the Vp2.
% マネキン関連説明
\begin{figure}[hbt]
\begin{center}
\includegraphics[width = 8cm]{figures/desc_mannequin.png}
\end{center}
\caption{
Schematic of the divisions of the mannequin to 3D print (a)--(b), and measurement conditions (c)--(e).
The letters in (a) and (b) indicate the dimensions: $a$ = 150 mm, $b$ = 62.5 mm, $c$ = 1100 mm, and $d$ = 70 mm.
The red and blue lines in (a) correspond to those in (b).
The green arrows in (c)--(e) indicate the direction of the x-axis of the accelerometer.
}
\label{fig:desc_mannequin}
\end{figure}
\par
\subsubsection*{\textbf{Result \& Discussion}}
\begin{figure}[hbt]
\begin{center}
\includegraphics[width = 8cm]{figures/mannequin_result.png}
\end{center}
\caption{
Result of the frequency responses of Hapbeat and Vp2 using the mannequin.
The blue line shows the amplitude of 10 $\mathrm{m/s^2}$.
}
\label{fig:mannequin_result}
\end{figure}
\par
The result shown in Fig. \ref{fig:mannequin_result} demonstrates that $ACC_{RMS}$ exceeded 10 $\mathrm{m/s^{2}}$ at 3.3 Hz for the housing, 4.7 Hz for the front, and 5.6 Hz for the side, and shows that Hapbeat can generate powerful vibrations from input signals below 10 Hz.
%
The Vp2 cannot output over 1 $\mathrm{m/s^{2}}$ below 20 Hz, demonstrating its unsuitability for low-frequency vibrations.
\par
% % 目的：筐体への組み込みによる影響が、触覚刺激の知覚に影響するどうかを検証する。胴巻き型との比較
\subsection*{Experiment 2: Comparing the Hapbeat and DC motor}
\par
% 消費電力と発熱について比較。目的：DCを使用しない場合にどれだけ消費電力や発熱量が減るかを調べるため。
\subsection{Comparing power consumption and heat generation}
\label{exp:powerConsumption}
We derived the power consumption with and without direct current (DC) to verify the contribution of the steady-state torque generated by the rubber cord to power saving.
% DC測定の手順
The measurement with DC (named the DC case) is determined as follows.
The Hapbeat includes two motors, and its weight is 58.5 grams plus connected cable mass. Thus, the tension applied on each motor will be about 0.3 N for regular usage.
With three rounds of thread wound on a bobbin, the thread was attached to a digital force gauge (Nidec-Shimpo Corporation, FPG-5) which measured the tension.
A power supply (Kenwood TMI Corp, PW18-1.8Q) applied voltage at which the motor generated 0.3 N of tension, and we then recorded the current.
% AC測定の手順
The measurement without DC (named the AC case) was conducted to derive the power consumption of regular usage.
Sub-6 wore the Hapbeat, and current values were measured three times when sine waves of 20Hz-1W, 80Hz-1W, and 140Hz-1W were input.
The power consumptions were calculated using $P=RI^{2}$ with the measurement values and the motor resistance of 1.1 $\Omega$.
\par
\subsubsection*{\textbf{Result \& Discussion}}
In the DC case, the motor current was 0.32 A.
In the AC case, the RMS current value derived from the average of three measurements was 0.65 A at 20 Hz, 0.92 A at 80 Hz, and 0.94 A at 140 Hz.
The results demonstrate that applying DC increases power consumption by 1.8--2.3 times compared with the AC case in driving the signal.
This will increase heat generation and decrease continuous running time.
\par
% 起動電流の際について検証・目的：起動電圧の値の違いが、触覚刺激の体験に影響を生じるかを検証。
\subsection{Comparing the starting current}
\label{exp:startingCurrent}
This experiment compared the starting current of the Hapbeat and DC motor to investigate the friction effect of the rubber cord and the Teflon tube.
A starting current is defined as a current value when the shaft rotates from a rest state in the DC motor case.
In the Hapbeat case, the starting current is defined as the current value when the thread first moves from rest.
The Hapbeat was suspended from a hook, with the accelerometer attached to the coupling using double-sided tape.
The accelerometer was used to detect the first move; its output was displayed on the oscilloscope.
\par
\subsubsection*{\textbf{Result \& Discussion}}
The result of 10 measurements shows the starting currents of the DC motor were all 0.01 A and that of the Hapbeat averaged 0.55 A (standard deviation was 0.02 A).
% % DC無しの電流実効値の結果から、これが影響あるかを論じる。
The voltage applied at the first move was 0.61 V in the Hapbeat case, indicating that a weak signal below 0.61 V cannot drive the Hapbeat from rest.
Note that the voltage amplitude applied to the motor at 20Hz-0.5W was 1.05 V.
\par
% % 筐体の重さを変化させた場合の、身体に伝わる振動について測定：（今回の組み込みが質量的に最小構成という前提で）適切な筐体質量を検討するため。
\subsection{Effect of the housing mass}
\label{exp:massEffect}
The steady-state tension of the Hapbeat, a necklace-type, depends on the housing mass which moves during the drive.
This is a big difference from the WTV, a body-wound type, and may affect the vibration transmission.
To examine the mass effect, we measured the transmitted vibration with weights attached to the housing.
Seal-type iron weights (19 mm wide, 12 mm long, and 3.5 mm thick) weighing 5 grams each were attached in units of four, and the measurements were taken three times for each total weight masses of 0, 20, 40, 60, 80, 100, and 120 grams.
The fifth and subsequent sheets were pasted on top of the attached weights.
The input signals were 20Hz-0.5W, 20Hz-1W, 20Hz-2W, 80Hz-1W, and 140Hz-1W.
The measurement points were at \#8 (the neck-side area) and \#6 (the nape area) of sub-6 wearing the underwear and T-shirt used in section \ref{exp:repeat_exp}.
\par
\subsubsection*{\textbf{Result \& Discussion}}
The neck-side result shown in Fig. \ref{fig:result_mass} demonstrates that $ACC_{RMS}$ of 78.5 grams in the housing mass was the largest at all input signals, and $ACC_{RMS}$ tended to decrease with increasing housing mass for 20 Hz signals.
Although $ACC_{RMS}$ of 80 Hz and 140 Hz input decreases at 98.5 grams, the decrease is not monotonic.
The nape result showed a similar trend to the neck-side, but to a lesser extent.
\begin{figure}[hbt]
\begin{center}
\includegraphics[width = 8.8cm]{figures/result_mass.png}
\end{center}
\caption{
Vibration transmission result with varying housing mass.
}
\label{fig:result_mass}
\end{figure}
\par
% 応答速度の測定
\subsection{Response time of the Hapbeat}
\label{exp:responseTime}
The response time of the Hapbeat was measured to examine whether the internal friction of the Hapbeat adversely affects the response time.
The Hapbeat hung on a hook-shaped part formed by the 3D-printer and was attached to the sensor tip.
The step voltage was applied by turning on a battery box that contained two 1.2 V AA batteries in series.
To normalize the measured data, the values before the step voltages were set to zero, and the average value of steady-state after the input was set to one.
The steady-state was defined as the voltage drifting within 0.1 V per second.
The time of interest was when the normalized value of the input voltage and tension increased from 0.1 and 0.9.
\subsubsection*{\textbf{Result \& Discussion}}
The average of ten trials was 2.74 milliseconds, and the maximum value was 3.00 milliseconds.
A previous study \cite{yem2016vibrotactile} has shown that the response time of a coreless DC motor is 3 milliseconds, and thus the result shows that the internal friction can be dismissed for the response time.
%6考察7限界
\section{General discussion}
The present study demonstrates that the proposed necklace-type device, Hapbeat, transmits low-frequency vibrations over a wide area of the user's body.
However, the transmitted vibrations contained a high percentage of harmonic components, even more than the inputted low-frequency component for some subjects.
\par
The subjective results demonstrate that most subjects clearly felt 20Hz-1W vibration at multiple locations in all the chest, neck-side, and nape areas, especially near the ribbon or housing.
This also indicates that the Hapbeat transmitted low-frequency vibration perceptually to a wider area.
The response time of the Hapbeat was 2.74 milliseconds, which is comparable to that of coreless motors or linear vibrators \cite{yem2016vibrotactile}.
The Hapbeat can also output high-frequency vibrations, exceeding 10 $\mathrm{m/s^{2}}$ up to 270 Hz, and the vibrations of 80 Hz and 140 Hz were perceivable near the ribbon or housing.
Our findings suggest that the Hapbeat is useful as a wearable vibroacoustic device because it covers a frequency range of 5--270 Hz, a low-frequency range in music, and can respond to impact sounds such as drums or explosions with slight delay.
\par
%%% 先行研究からのメリット
We also succeeded in redesigning WTV as a necklace-type device to improve usability, developing a drive circuit that can draw a high current with audio signals and a battery, and saving power consumption using a rubber cord to generate a steady-state torque.
This means the Hapbeat is easy to wear (takes less than five seconds to wear) and can be used anywhere, whereas WTV requires a power source to drive, a structure to fix, and a long time (more than ten seconds) to wear.
\par
We describe some interesting findings from the experiments in the following subsections.
%% 服の比較
\subsection{Effect of clothing}
Comparing the transmitted vibrations to the T-shirt and dress shirt from Fig. \ref{fig:result_trans_subject}, the dress shirt more effectively transmitted the vibrations to a wider area in both quantitative and subjective results.
This may be due to the higher Young's modulus of the dress shirt fabric.
The $ACC_{RMS}$ of the housing (\#22) was also larger for the dress shirt, suggesting that the T-shirt easily deformed and prevented housing movement due to its softness.
These results indicate that clothes will affect the vibration transmission from Hapbeat, and clothes with a higher Young's modulus may transmit more effectively.
This phenomenon may occur with other general vibrators attached to clothes.
\par
\subsection{Vibration propagation by skin surface waves}
The result of the T-shirt neck-side in Fig. \ref{fig:result_ampfreq_comparison} shows the $ACC_{RMS}$ at \#6, 7 cm away from the ribbon, greatly attenuated than that of \#8, near the ribbon.
The vibration transmission of internal skin from the vibrating source to a distant point is known to occur by shear waves, which are primarily through soft tissue in the frequency range of tactile perception \cite{moore1970survey}.
Dandu et al. \cite{dandu2019spatiotemporal} performed a Fourier expansion of the polarization for an arbitrary plane and presented the equation below for the skin strain vector from the following findings: the equation of motion for elastic bodies, the damping rate and transport rate of viscoelastic skin and soft tissue dependent on the vibration frequency \cite{manfredi2012effect}, \cite{pereira1991dynamic}, and the solution of strain vectors for time and distance from a vibrating source in soft tissue in a linear viscoelastic model.
\begin{equation*}
\xi ( x,t) =\int ^{\infty }_{-\infty } df\ \phi ( f) \ e^{-\alpha xf} \ e^{j2\pi f( x/c( f) \ -\ t)}
\label{eq:kai}
\end{equation*}
where $\xi(x,t)$ is the time-varying strain vector, $\phi(f)$ is the amplitude and phase of a frequency component $f$, $x$ is the distance from the vibrating source, $t$ is time, and $c(f)$ the propagation velocity.
In the linear viscoelastic model, the damping is considered to increase almost linearly with frequency, so the damping rate is assumed to be $\sigma = \alpha f$ (where $\alpha$ is an arbitrary constant).
From this, it can be seen that the vibrations decay exponentially with increasing distance and frequency.
\par
This phenomenon aligns with the results obtained in the experiment; the higher input frequency occurs with lower damping percentage as shown in Table \ref{tab:dampingRate}, indicating that skin viscosity damped the vibration.
The subjective result of Fig. \ref{fig:result_ampfreq_comparison}, in which the subjects only felt vibration near the ribbon, also support this.
The damping percentage slightly decreases as the output increases, but the subjective results are almost the same.
The reason can be that the transmitted vibration of 20Hz-0.5W was easily perceptible, and the increased values of $ACC_{RMS}$ at distant locations were relatively smaller than near the ribbon.
Additionally, in all cases, the subjects hardly felt the vibrations at \#6, 7 cm from the ribbon.
\par
The findings indicate that expanding the contact area of the vibrating part achieves more extensive transmission than increasing the vibration output.
This confirms that the proposed method, in which a ribbon is contacted widely to a user's body to actuate the skin, is suitable for extensive transmission.
\par
%% デメリット。立ち位置的にLimitationか。
\section{Limitations}
The outputs of the low-frequency vibration contained a high ratio of harmonics, which resulted in poor reproducibility of the input signal (Fig. \ref{fig:result_fft}).
Because the Hapbeat is suspended, it cannot actuate the user's skin when it unwinds and loosens the thread.
Thus, the Hapbeat discards the negative voltage part of input signals if we define the positive voltage as it drives the motor to wind the thread.
The internal friction, derived from the contact between the thread or rubber cord and the Teflon tubes, stops thread movement occurring with a weak input voltage.
This leads to a rapid and intense actuation when the input voltage exceeds a certain value.
These phenomena may have caused the spike waveform of the vibrations transmitted from the Hapbeat, as shown in Fig. \ref{fig:result_fft}, resulting in a high percentage of harmonics.
\par
The result of the experiment in section \ref{exp:massEffect} shows that the housing mass affects vibration transmission.
This implies that changing the steady-state tension could control the transmission characteristics, e.g., emphasizing high-frequency vibrations or vibrations transmitted to the nape area.
However, the steady-state tension of the Hapbeat is difficult to control because it depends on the housing mass.
The 20 Hz vibrations decreased when the housing mass exceeded 78.5 grams.
The larger steady-state tension, caused by heavier housing mass, maximally stretches the rubber cord and limits the maximum angular displacement of the bobbin.
This limitation possibly causes the decrement, considering actuating low-frequency vibrations requires a longer stroke of actuators.
Increasing the rubber cord length can solve the problem, but it will cause other problems such as increasing the housing volume or internal friction.
\par
% 実験手法のLimitation
The subjects of the experiments were only six males, and transmitted vibrations at some measurement points showed quite large individual differences.
Thus additional experiments, considering more conditions such as subjects' body shape and the contact state of the ribbon, are needed to derive a general vibration transfer function for the Hapbeat.
\par
% 振動伝達だけ考えれば巻き付け＆DCによる定常張力の方が好ましい
These negative results indicate that Hapbeat is an unsuitable device for transmitting vibration fidelity from an input signal.
The following modifications, which improve the usability, will increase the number of factors that affect the transmission: using a rubber cord to generate steady-state tension, incorporating the mechanism into the housing, and wearing a device like a necklace.
Therefore, generating a steady-state torque by DC motors as in the WTV is better for transmitting vibration fidelity.
% 体感音響ではエンベロープが周波数より重要(?)
\par
However, the main usage of Hapbeat is the vibroacoustic effect.
Auditory researches have shown that a brain tracks the envelope of speech and music \cite{di2020cortical}, \cite{cantisani2019eeg}.
This fact may imply that a device used for the vibroacoustic effect is required to have envelope fidelity rather than frequency fidelity.
% そもそも服による（悪？）影響の方がWTV➡Hapbeatになる影響よりも大きいのでは
In real-life use, the effects of clothing type will have an impact on transmission.
Thus, additional experiments are required to determine the extent to which the disadvantages will affect the perception of the vibroacoustic effect.
%8結論
\section{Conclusion}
This paper proposed a necklace-type haptic device, Hapbeat, and the experimental results demonstrated that it could transmit high-power, low-frequency vibrations over a wide area.
The results also show the response time is comparable to linear vibrators, and the Hapbeat can output easily perceptible vibrations from a 5--270 Hz sine wave input.
Thus, our proposed method enables a small vibroacoustic device that can transmit powerful low-frequency vibrations over a wide area, which is difficult to achieve with conventional devices.
Although this paper focused on the necklace-type, the method can be applied to various wearable haptic devices such as belt-type or wristband-type.
The vibroacoustic effect is a special experience that can only be felt in certain facilities or limited environments.





































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































































==> Don't use/sub1-intro.tex <==
\section{Introduction}
The vibroacoustic effect, which plays a vital role in enhancing the experience of music, movies, and other entertainment content, is mainly due to air pressure changes from the sound source acting on the entire body directly or via a solid object.
This haptic sensation can be felt from sources such as the heavy bass from the large sub-woofers installed in live-music venues, clubs, and cinemas, the blooming of fireworks, and the sounds of gunshot and bombing in maneuvering grounds.
The feeling is difficult to create in daily life owing to the cost of equipment and loud noises. Although recent technological developments enable the enjoyment of the entertainment events remotely, many people still opt to attend in person \cite{liveMusicRevenue}.
To overcome these challenges, researchers are developing a way to display vibroacoustic sensation using haptic devices with vibrators, contributing to the enhancement of the immersive experience of such content \cite{karam2010emoti}, \cite{konishi2016synesthesia}, \cite{subpac}, \cite{woojer}, \cite{bhaptics}.

However, many small vibrators or few large vibrators need to be embedded in the devices to achieve a wide range of vibration transmission. Consequently, such devices should be large, expensive, and uncomfortable to use.
The mechanism of the eccentric motor and linear vibrators, including the general speaker, commonly used in general haptic devices, cause the size and expense (Fig. \ref{fig:desc_vibration_mechanism} left).
All of these general vibrators use the reaction force by moving the internal weight.
To increase the output in the ultra-low frequency band (below 20 Hz), an essential band for vibroacoustic effect, the mass and stroke of the internal weight, in terms of momentum, need to increase.
This mechanical requirement causes the challenging trade-off between the device size and high-power low-frequency vibrational output.

The high-frequency band in the tactile domain, the sensitive band of the Pacinian corpuscle \cite{sato1961response} (100 to 1000 Hz), also cannot be underestimated.
The experiment held by Merchel et al. \cite{merchel2013music} revealed that vibrations of high frequency from the speakers located at the stage of the concert hall reached the audience seats.
"The response speed is also important. 
Previous studies on the synchronization of auditory and tactile stimuli have shown that asynchrony can be distinguished in about 20–50 milliseconds \cite{adelstein2003sensitivity}, \cite{balandra2019sensitivity}, \cite{levitin2000perception}, so the delay of vibrators should be less than this value."

"Our previous study proposed a vibration generation mechanism using motors and a thread (Fig. \ref{fig:desc_vibration_mechanism}(b)) that solves the trade-off \cite{yamazaki2016tension}. 
We developed and evaluated a body-wound-type prototype called Wearable Tension-based Vibroacoustic Device (hereafter referred to as WTV) shown in Fig. \ref{fig:desc_vibration_mechanism}(c))."
"The study has demonstrated that a small device can transmit powerful low-frequency vibration over a wide area in principle.
However, the principle prototype has several problems in terms of practical usage.
The winding-type prototype is troublesome and discomfort to wear, and the actuators consume high electricity, which heat them up extremely and increase the size of a driver circuit."

"This study aims to demonstrate a practical wearable device using our mechanism can transmit low-frequency vitration over a wide area of the user's body.
We developed a necklace-type device called Hapbeat
\footnote{
We originally named ""Hapbeat"" to any haptic device using one or more motors and threads, and Hapbeat can form not only a necklace-type. However, we define ""Hapbeat"" as a necklace-type in this paper for clarification.
}
 and tested (1) the performance of vibration transmission on the user's body and (2) the fidelity of vibration waveform compared to input signals. "
To show the usage of our mechanism, we also list key elements to be considered in downsizing and tested the characteristics of a necklace-type device compared to a body-wound-type device.

\begin{figure}[hbt]
\begin{center}
\includegraphics[width = 8cm]{figures/desc_vibration_mechanism.png}
\end{center}
\caption{
"The mechanism of (a) direct-acting transducer and (b) proposed mechanism. The red arrows indicate actuator movement, and the blue arrows indicate the movment driven by the actuator. 
The blue and green dots in the top and sectional view correspond to each other and indicate the max and minimum state of the output for the sinusoidal wave input.
$r$ stands for the distance between the thread to be reeled out and the center of the bobbin, which can be approximated to the inner radius of the bobbin.
(c) The body-wound-type prototype proposed in our previous study."
}
\label{fig:desc_vibration_mechanism}
\end{figure}


==> Don't use/sub2-relatedworks.tex <==
\section{Related Works}
Much research has been accomplished on the transmission of vibrations to a wide area of the human body to enhance the experience of entertainment content.

% 小型振動子デバイスの説明 
For example, previous studies proposed clothing-type and chair-type haptic devices embedded with several small vibrators to directly stimulate any part of the body \cite{konishi2016synesthesia}, \cite{lemmens2009body},  \cite{chandra2020preliminary}, \cite{israr2012surround}, \cite{5196671}.
These haptic devices are suitable for conveying complex information such as distance or direction by stimulating arbitrary areas because of their high spatial resolution.
However, small vibrators cannot sufficiently output low-frequency vibration, and incorporating more vibrators would increase manufacturing costs and risks.

% 大型振動子デバイスの説明 
In addition, there are other haptic devices that have only a few large vibrators embedded in the back of a chair or a backpack \cite{karam2010emoti}, \cite{subpac}, \cite{woojer}, \cite{nanayakkara2009enhanced}.
"These devices have a low spatial resolution, but their large contact area contributes to the transmission of the vibrations over a wide area of the user’s body.
It can also play stronger low-frequency vibration compared to small vibrators because the mass and stroke of the internal weight are larger.
"
This type of haptic device is thus suitable for displaying the vibroacoustic effect, typically encountered when watching movies or listening to music.
However, portability is not an option owing to the device size.
"Consequently, the chair-type device has restrictions on location and posture, and the backpack-type device has limitations due to the load, such as weight and tightness.
The heavy internal weight also sacrifices response speed and high-frequency output, and the components such as the chair or the backpack increase the overall cost of the device.
"

% 工夫した例の説明 
Some studies have proposed different approaches to efficiently transfer the vibration over a wider area.
Sakuragi et al. used bone conduction and showed that a clavicle can effectively be attached to a vibrator \cite{sakuragi2015collarbeat}.
Kurihara et al. incorporated particles of granular Styrofoam as a medium to convey vibration evoked from an audio speaker to the contact area \cite{kurihara2014large}.
Anusha Withana et al. applied properties of low-frequency acoustic wave propagation in the human body and proposed a low-resolution haptic interface that is capable of providing haptic stimulation to multiple areas of the body via a single-point-of-contact actuator \cite{withana2015rippletouch}.
These approaches involve vibration transmission through an object, which allows for a larger transmission area with fewer vibrators and a simpler device compared to the devices mentioned earlier.
However, the vibrators in these applications are conventional and do not, therefore, resolve the aforementioned trade-off.

% モーターをアクチュエータとして利用した例
In contrast, Yem et al. \cite{yem2016vibrotactile} show that DC motors are effective vibrators capable of driving low-frequency vibrations by harnessing the rotational motor’s counter force and using the rotor of the motor as the vibration mass.
"In addition, Minamizawa et al. \cite{minamizawa2007gravity} and Nakamura et al. \cite{nakamura2017hapbelt} used a belt in contact with a fingertip and a rotational motor as a driver.
The deformed skin artificially presented the sensations, such as holding an object or the feeling collision and traction in a video game."
"The rotational motion of the motor shaft, as the source of vibration, is ultimately converted into a translational motion of the skin.
The skin displacement can be increased, and static forces and low-frequency vibrations can be effectively represented."
However, these studies focus on the fingertips, i.e., a localized area, and differ from the purpose of this paper, which is to transmit vibrations over a wide area.


==> Don't use/sub3-proposal.tex <==
\section{Proposal}
We propose a compact necklace-type haptic device that can transmit high-power low-frequency vibrations to a wider area of the user’s body using our proposed mechanism (Fig. \ref{fig:desc_vibration_mechanism}(b)).

% 課題の解決説明
"As described in the related works, the challenges of current haptic devices are their heaviness, large size, and inability to produce high-power, low-frequency vibration output over a wide area.
This is because they used eccentric motors or linear vibrators."
Our previous work \cite{yamazaki2016tension} demonstrated the proposed mechanism transmits high-power lower-frequency over the wide-area independent of the device size, and thus using the mechanism can solve the challenges.
Here, we explain the proposed mechanism (Fig. \ref{fig:desc_vibration_mechanism}(b)) and prototype (Fig. \ref{fig:desc_vibration_mechanism}(c)) in our premvious study.
The bobbin is attached to the shaft, and the thread is tied to the bobbin.

"The other end of the thread is wound around the bobbin several times and then rolled out of the enclosure.
The thread is wound around the user’s body and then similarly wound and fixed to another bobbin attached to a motor shaft located on the opposite side."
"Thus, the rotational movement of the shaft is converted into a translational movement of the thread.
The area of the body in contact with the thread is actuated, thereby transmitting vibration."
The thread is wound onto the bobbin, and thus the maximum stroke amplitude is determined by the bobbin capacity and the thread volume.
The volume is relatively small compared to the capacity of the bobbin, making it possible to generate high-power low-frequency vibrations in a small enclosure.


% ベルト型からネックレス型に変更した理由
"In a previous study \cite{yamazaki2017hapbeat}, we developed a belt-type device using this mechanism to improve the music listening experience and demonstrated at an exhibition.
However, the attendees noted the following problems with convenience."
First, each time after putting the belt-type device on the body, tightness needs to be obtained by adjusting the length of the belt, a tedious task that takes more than ten seconds.
Second, the transmitted vibration gets weaker when worn over thick clothing, and in some cases, the users needed to take off or roll up the dress.
Third, the tightness on the body causes a sense of pressure, which is not suitable for long-time use.
A necklace-type device does not require adjustment of the ribbon length, and the users only have to suspend it from the neck.
Suspending the device puts little pressure on the users, and the device rarely interfere with the users' movement.
This makes a necklace-type device suitable for long-time use in daily life.

==> Don't use/sub4-implement.tex <==
\section{Implementation}
\label{inplementation}
The structure and components of Hapbeat are shown in Fig. \ref{fig:desc_hapbeat_mechanism}.
\begin{figure}[hbt]
\begin{center}
\includegraphics[width=7cm]{figures/desc_hapbeat_mechanism.png}
\end{center}
\caption{
"The description of the structure and components of Hapbeat. 
(a): The value of $\rho$ indicates the curvature radius of the tube.
(b): The green arrows indicate the direction of the tension applied to the bobbin when the thread is reeled out.
(c): The dimensions of the bobbin. The $\phi$ indicates the diameter of the corresponding part."
}
\label{fig:desc_hapbeat_mechanism}
\end{figure}
The volume is roughly 38 $\mathrm{cm^3}$, the mass is 58.5 g, and the maximum thread feed length, which corresponds to the full stroke length, is approximately 50 mm.
The enclosure and bobbin were formed by an industrial 3D-printer (HP Development Company, L.P., HP Jet Fusion 4200, PA12).
For implementation, a rigid thread, a coreless motor, and a steady torque are required.
"Although a belt, as used in related works \cite{minamizawa2007gravity}, \cite{nakamura2017hapbelt} could transmit the vibration, we adopted a polyethylene line as the thread component (RUNCL PowerBraid [four strands, 95 lb / 0.50 mm, gray]).
It is rigid and thus effectively reflects the shaft's movement; it is easy to store inside the bobbin, contributing to downsizing and weight reduction."
"Additionally, a satin ribbon (6-mm wide, 100\% polyester) is used for contact component to the user's body.
The ribbon is connected to the thread by plastic couplings."
The motor should be coreless with a low moment of inertia to transmit vibration to allow quick repetitions of forward and reverse rotation.
The coreless motor used in Hapbeat was ordered with the following characteristics: 3-V rated voltage, 1.1-$\Omega$ armature resistance, 1.92-W max output, 6.8-mNm stall torque, 10-ms mechanical time constant, 0.6-$\mathrm{G \cdot cm^2}$ rotor moment of inertia, 110-$\mathrm{10^3rad/s^2}$ angular acceleration.

% 定常張力の説明
\subsection{Implementation of steady-state torque}
To properly convert a signal applied to the motor into translational motion, the thread must be sufficiently wound on the bobbin while suspended from the user’s neck.
For this reason, generating a steady-state torque is necessary to prevent the thread from unrolling off the bobbin.
Applying an offset voltage to the motor is desirable in terms of simplicity and waveform fidelity but not practical because of the increase in power consumption, heat generation, and deterioration of the motor.
"Instead, a rubber cord (KawamuraSeichu Co, Ltd, Elastic cord 1-mm diameter white, made of natural rubber and rayon, 36-mm length) was used as a  spring material, which combines thinness and high elongation rate.
One end of the rubbor cord was fixed to the bobbin and the other end to the enclosure, applying counter-torque when the thread is unrolled from the bobbin (please refer to the green arrow in the Fig. \ref{fig:desc_hapbeat_mechanism}.)"
For this purpose, the bobbin has three flanges (Fig. \ref{fig:desc_hapbeat_mechanism}(c)).

\subsection{Incorporate into the housing}
\label{Incorporate}
For practical use, exposing the motor should be avoided from the risk of burns due to its heat generation, and thus the motor is incorporated in the housing.
Minimizing the friction of the threads and rubber should be considered to keep the efficiency of vibration transmission.
Teflon tubes (CHUKOH CHEMICAL INDUSTRIES, LTD. PTFE tube, inner diameter $\times$ outer diameter is 1 mm $\times$ 3 mm for the string and 1.5 mm $\times$ 2.5 mm for the rubber cord) guide them.
The tubes bend to minimize the housing, as shown in Fig. \ref{fig:desc_hapbeat_mechanism}, and the curvatures of them form as large as possible to reduce the friction.
For the connection between the motor and a drive circuit, a general stereo mini-jack is used for compatibility and soldered to the motor terminals.

\subsection{Circuit design}
\label{imp:circitDesign}
Using Hapbeat anywhere should be driven by a battery and is desirable to be recharged with a general 5-W output USB charger.
"A commercial audio amplifier can drive Hapbeat, which is driven by audio signals. 
However, Hapbeat requires a high current of more than 1 A, i.e., a 20-W output class amplifier is required, which is inconvenient."
"Thus, we designed a circuit of Hapbeat, which can draw a high current with audio signals and a battery. 
"
FETs (TPC8408, TOSHIBA ELECTRONIC DEVICES \& STORAGE CORPORATION) connected to the output of class-D amplifier IC (PAM8403, Diodes Incorporated) reduce the output impedance.
Additionally, general audio amplifiers cut off frequencies below 20 Hz to improve sound quality, unsuitable for Hapbeat.
"To lower the cut-off frequency, we adjusted parameters of resistors and capacitors, which form a high-pass filter at the input of the amplifier IC: the resistors were set 10 $\mathrm{k\Omega}$, and the capacitors were set to 2.2 $\mathrm{\mu F}$, resulting in the cut-off frequency of 7.2 Hz.
"
%% 回路図は無くても良いのでは？指摘されたら足す。
% 該当部分の回路図を図\ref{fig:desc_schema}に示す。
% \begin{figure}[hbt]
% \begin{center}
% \includegraphics[width = 7cm]{figures/desc_schema.png}
% \end{center}
% \caption{Schematic of designed driver circuit focused on driving part.}
% \label{fig:desc_schema}
% \end{figure}

\subsection* {Evaluation of the driver circuit}

We compared the performance of the designed circuit and a commercial audio amplifier (LP-V3S, Lepy. 25-W output. Hereafter referred as Lepy) in terms of frequency response and total harmonic distortion (THD).
"Input signals were sine waves of 0.5-V amplitude at frequencies based on the E12 series values (1.0, 1.2, 1.5, 1.8, 2.2, 2.7, 3.3, 3.9, 4.7, 5.6, 6.8, 8.2, these values times 1, 10, 100 for a total of 37 types from 1 to 1000 Hz).
A function generator (FY6600-30, FeelTech.) inputted the signals to the designed circuit and Lepy.
"
"An oscilloscope (MDO4024C, TEKTRONIX, INC.) recorded the output signals from the deigned circuit and Lepy with the sampling rate of 1 kHz for 1--8.2 Hz input and 10 kHz for over 10-Hz input.
The measurement was conducted three times with the maximum volume of the designed circuit and Lepy. "
The THDs were calculated by the "thd" functions of MATLAB (The MathWorks, Inc. version R2021b) with the harmonic number of six.
\begin{figure}[hbt]
\begin{center}
\includegraphics[width = 8cm]{figures/result_amp_comparison.png}
\end{center}
\caption{
Frequency response result of the designed circuit and Lepy.
The maximum standard deviation of the gain is 0.011 dB for both amplifiers, and that of the THD is 0.72 dB for the Hapbeat and 1.22 dB for Lepy.
}
\label{fig:result_amp_comparison}
\end{figure}

\subsubsection*{\textbf{Result \& Discussion}}
The result is shown in Fig. \ref{fig:result_amp_comparison}.
"Although the designed circuit is battery-powered, it showed better performance than Lepy in 1--22-Hz input.
This indicates the designed circuit is more suitable for driving Hapbeat, which is good at driving input signals below 20 Hz."


==> Don't use/sub5-evaluation.tex <==
\section{Evaluation}
In the experiment 1, we measured the transmitted vibration on subjects to verify the Hapbeat can transmit low-frequency vibration over a wide area.
In the experiment 2, we investigated the power consumption, the starting current, the effect of the Hapbeat enclosure mass, and the response speed to input to evaluate the effect of altering the device form from body-wound-type (WTV) to necklace-type (Hapbeat).

% 身体への振動伝達、複数回実施。目的1：Hapbeatの低周波振動が広範囲に伝わっていることを確認。被験者実験を行う際にどの測定点で測定するのが妥当かを検証
\subsection*{Experiment 1: Vibration transmission to the subjects' body}
\subsection{Detailed examination of vibration transmission}
\label{exp:repeat_exp}
In this experiment, the transmitted vibrations were measured at 71 locations on one subject (30-years-old male, 174-cm height, 74-kg weight, and 24.3\% body fat) to determine the necessary and sufficient measurement locations for evaluating the vibration transmission.
The measurement locations were placed as shown in Fig. \ref{fig:desc_position}, dividing the area into three sections: the chest, neck-side, and nape.
Hereafter, the measurement points are written by numbers with a hash tag, e.g., \#4 shows the measurement point 4 in Fig. \ref{fig:desc_position}.
\begin{figure}[hbt]
\begin{center}
\includegraphics[width = 8cm]{figures/desc_position_v2.png}
\end{center}
\caption{
Location of measurement points.
The blue numbers are identification numbers of measurement points in each area.
The magenta framed identification numbers indicate the measurement points on the clavicle or stitch.
The black numbers show the length in millimeter, and the blue numbers identify the points.
The green measurement points are extracted points used in \ref{exp:subject_exp}.
The red circled letters are reference points in each row, determined by the following criteria: A: contact point between the ribbon and the clavicle; B: middle point between A and C; C: center of the coupling; D: the middle point of the housing; E: cross point between the ribbon and the stitch extension line; F: center of the cervical vertebrae (approximate).
}
\label{fig:desc_position}
\end{figure}
The voltages of input sine waves from the function generator were adjusted to consume 0.5 W, 1 W, 2 W at 20 Hz, and 1 W at 80 Hz and 140 Hz by one motor.
Hereafter, the signal types are expressed as [frequency]-[power consumption], e.g., 20Hz-1W shows the input signal with a frequency of 20 Hz and a voltage adjusted to consume 1 W by one motor.
"The transmitted vibration from the Hapbeat was measured with an analog triaxial accelerometer (MMA7361LC, NXP Semiconductors, using 6 G mode).
"

"Considering the casual scene as a use case of Hapbeat, the subject wore a T-shirt or dress shirt and underwear.
The description of the clothes are shown as follows: the T-shirt (U CREW NECK SHORT-SLEEVE T-shirt WHITE, UNIQLO Co. The following clothes are all made by UNIQLO), the dress shirt (MEN EXTRA FINE COTTON BROADCLOTH LONG-SLEEVE SHIRT WHITE 100\% Cotton), and underwear (AIRISM MICRO MESH V-NECK SHORT-SLEEVE T-shirt WHITE 83\% Nylon, 17\% Spandex)."
The friction coefficients and Young's moduli of the T-shirt and dress shirt are shown in the table \ref{tab:clothing}.

\begin{table}[]
\centering
\caption{Friction coefficient and Young's modulus of the clothing}
\label{tab:clothing}
\scalebox{1}
{
\begin{tabular}{rl|cc}
Clothing    & Direction  & \begin{tabular}{c} Friction \\ Coefficient \end{tabular}
& \begin{tabular}{c} Young's \\ modulus \end{tabular} \\ \hline
T-shirt     & Vertical   & 0.188                & 573 $N/mm^2$    \\
& Horizontal & 0.203                & 546 $N/mm^2$ \\
Dress shirt & Vertical   & 0.179                & 17.6 $N/mm^2$ \\
& Horizontal & 0.178                & 11.0 $N/mm^2$
\end{tabular}
}
\end{table}

The friction coefficients were measured by a surface tester  (KES-FB4-A, KATO TECH CO., LTD.)
A 20 $\times$ 20 cm sample was prepared and tested six times using 400 g weight (used for applying tension on the sample), and the average value was calculated.
Young's moduli were measured by a tensile tester (RTF-1250, A\&D Company, Limited).
"The tensile test was performed according to the Tensile Test of Fabrics (JIS L 1096 Strip Method).
Five samples were cut out from the T-shirts' vertical and horizontal direction, and three from the dress shirts' vertical and horizontal direction, respectively.
Each sample dimension was 50 $\times$ 300 mm, and the grepping interval during the test was 200 mm.
Tests were conducted on each sample, and the average values were then calculated. "

"For comparison with Hapbeat, we used a Vp2 (Vp210, Acouve Laboratory, Inc.) as a representative of linear vibrators.
The transmitted vibrations from the Vp2 were measured at the points on the red line in Fig. \ref{fig:desc_position}."
"The signals of 20Hz-2W, 80Hz-2W, and 140Hz-2W were inputted to the Vp2 by the Lepy.
The input signal voltage was set to consume 2 W by the Vp2 to match the total power consumption of the Hapbeat, consists of two motors."
A rubber belt (KIYOHARA \& Co., Ltd., SUN40-163, made of LYCRA percent elongation is 120\%, 25cm width, white.) with a buckle attached the Vp2 on the subject.
"The length of the rubber belt, including the buckle, was determined as follows.
The Vp2 was temporarily attached to the subject using a double-sided tape (AD\&F WIG double-sided hard tape, Aderans Co., Ltd) at the same location as the Hapbeat in Fig. \ref{fig:desc_position}.
Then the circumference of the subject's body, including the attached Vp2 height, was measured.
The 75\% of the measured circumference became the rubber belt length."

\subsubsection*{\textbf{Procedure}}
Initially, the measurement points were marked on the subject’s body with a pen, as well as an outline of the enclosure, so that it could be restored to the initial place if the Hapbeat was misaligned during the experiment. 
"The accelerometer was then attached to the measurement point with its x-axis parallel to the green and yellow arrows in Fig. \ref{fig:desc_position} and z-axis perpendicular to the body surface.
To maintain the attachment, an experimenter held the accelerometer cable 20-cm apart from the sensor part."
At each measurement point, measurements were made once for input signals of 20Hz-0.5W, 20Hz-1W, 20Hz-2W, 80Hz-1W, and 140Hz-1W, respectively.
The subject stabilized his posture during the experiment by following these instructions: sit on a chair with your upper body perpendicular to the seat surface, lightly press your back and head against the pole fixed directly behind the chair, keep your eyes at the same level throughout the experiment (level with an object in the room).
These procedures was conducted three times for the T-shirt and dress shirt.

\subsubsection*{\textbf{Result \& Discussion}}
The results are shown in Fig. \ref{fig:result_trans_repeat}.
Hereafter, we evaluate the magnitude of the transmitted vibration by root-mean-square values of measured accelerations designated as $ACC_{RMS}$ derived from eq. (\ref{eq:value}).
\begin{equation}
ACC_{RMS}\ =\ RMS_{x} +RMS_{y} +RMS_{z} \label{eq:value}
\end{equation}
\begin{equation}
RMS_{x} =\sqrt{\frac{1}{N}\sum\limits _{n=1}^{N} |x_{n} -\mu |^{2}},
\;\;\; \mu \ =\ \frac{1}{N}\sum _{n=1}^{N} x_{n}   \label{eq:rms}
\end{equation}
Where $x_{n}$ is a sampled data, $N$ = 10 k (points), eq. (\ref{eq:rms}) is same for y-axis and z-axis.
"Selected measurement points used in the experiment \ref{exp:subject_exp} are shown as green points in Fig. \ref{fig:desc_position}.
The reasons for the selection are described below."
For the chest and neck-side area, we selected the points only located on the right side because both sides' $ACC_{RMS}$ and attenuation tendency seemed similar. Investigating the asymmetry is out of our purpose.

For the neck-sides and nape area, we first selected all points located near the ribbon because the large $ACC_{RMS}$ indicated importance for perception.
"Then we selected center points located far from the ribbon because the $ACC_{RMS}$ of the skin points at the same distance from the ribbon ( e.g., \#2, \#7, and \#12 in the neck-side area) differed within only $\pm 0.071 \mathbf{m \cdot s^{-2}}$ at most.
Additionally, the large-small relationships among those points seemed similar to those of points near-ribbon points."

"For the points near the ribbon in the chest area, we selected \#11 to \#13 rather than \#15 to \#17.
The trends were similar, and we wanted to observe the vibration damping."
For the rest points, we selected them to observe vibration damping. The clavicles (\#1, \#6, \#10) may reflect the effect of body shape. The damping trends from the housing (\#5, \#10, \#14) and the clavicle or coupling contact (A and C in Fig.\ref{fig:desc_position}) may differ from other points.
\begin{figure*}[hbt]
\begin{center}
\includegraphics[width = 17cm]{figures/result_trans_repeat.png}
\end{center}
\caption{
Result of the vibration transmission conducted on the single subject (sub-6).
The circles' sizes indicate the magnitude of $ACC_{RMS}$ and the colors indicate input signal type.
}
\label{fig:result_trans_repeat}
\end{figure*}

The result of Vp2 shown in Fig. \ref{fig:result_Vp2_repeat} demonstrates the Vp2 transmits larger $ACC_{RMS}$ than the Hapbeat at 80 Hz and 140 Hz, but almost no vibration at 20 Hz.
\begin{figure}[hbt]
\begin{center}
\includegraphics[width = 8cm]{figures/result_Vp2_repeat.png}
\end{center}
\caption{
Results of the acceleration measurement wearing a Vp2.
}
\label{fig:result_Vp2_repeat}
\end{figure}

% 複数の被験者での振動伝達実験。目的：色々な体格の装着者でも、実験\ref{sec:repeat_exp}と同傾向の結果（振動伝達範囲、服による傾向）が得られるかを確認する。
\subsection{Vibration transmission on various body type}
\label{exp:subject_exp}
We conducted vibration propagation experiments with six subjects of different body sizes to verify that Hapbeat can extensively transmit powerful low-frequency vibration, even among users with various body types.
The subjects' height, weight, and body fat percentage values measured with a body composition meter (innerScan Dual RD-802, TANITA CORPORATION) are listed in the table \ref{tab:subject_info}.
The subjects were named sub-1 to sub-6 in ascending order of body fat percentage.

% 被験者の情報テーブル
\begin{table}[hbt]
\centering
\caption{
Information of subjects
}
\label{tab:subject_info}
\scalebox{1}
{
\begin{tabular}{r|cccccc}
& sub-1 & sub-2 & sub-3& sub-4 &sub-5 & sub-6 \\ \hline
Height (cm)              & 185  & 160  & 164  & 165  & 178  & 174  \\
Weight (kg)              & 61.8 & 47.3 & 52.4 & 56.8 & 61.1 & 74.1 \\
body-fat (\%) & 12.1 & 12.3 & 16.9 & 18.7 & 18.8 & 24.3
\end{tabular}
}
\end{table}

"The experimental procedure was the same as in the experiment \ref{exp:repeat_exp}. 
However, to shorten the experimental time, the measurement points were limited to the green points in Fig. \ref{fig:desc_position} for the reasons described in the results of experiment \ref{exp:repeat_exp}. 
One measurement was taken per subject."

We also evaluated the subjective vibration perception for each input signal.
"The subjects colored measurement points in a figure---Fig. \ref{fig:desc_position} with all explanatory numbers and letters omitted and all points colored black---with the following criteria: (1) red color where subjects clearly felt the vibration, and (2) blue color where subjects subtly felt the vibration.
The difference between the clear and subtle is whether they need concentration to percept the vibration."
Initially, the experimenter touched the measurement points on the subjects' body to make them recognize the locations.
During the experiment, the Hapbeat continuously vibrated subjects. 
No time limit was set for the evaluation, but the subjects were asked not to touch their bodies.

\subsubsection*{\textbf{Result \& Discussion}}
\begin{figure*}[hbt]
\begin{center}
\includegraphics[width = 18cm]{figures/result_trans_subject.png}
\end{center}
\caption{
Result of the vibration transmission conducted on the six subjects.
"The six columns of squares located above the bars indicate the result of the subjective experiment.
Fulfilled squares indicate the subject clearly felt the vibration, and half-filled squares indicate the subject subtly felt the vibration."
The red-colored numbers indicate the point 1 cm away from the ribbon or housing, and the underlined numbers indicate the points measured on the skin.
}
\label{fig:result_trans_subject}
\end{figure*}
The result of vibration transmission is shown in Fig. \ref{fig:result_trans_subject} demonstrates that the Hapbeat transmitted powerful 20-Hz vibrations, $ACC_{RMS}$ of 10 $\mathrm{m \cdot s^{-2}}$ or greater, to the subjects' skin and clothing across the chest, neck-sides, and nape areas.

% TシャツとYシャツの比較
Comparing the results of the T-shirts and dress shirts, overall $ACC_{RMS}$ of the dress shirts were greater than that of T-shirts.
This is seemingly due to the larger Youngs' modulus of the dress shirt.
% 被験者ごとによって大きく異なる
The $ACC_{RMS}$ on some measurement points differed greatly depending on the subjects.
This is seemingly due to the difference in wearing condition and subjects' body type.

%% 主観実験について
% 前面、筐体・結合部付近で知覚が強い。
The subjective result in the dress shirt chest area shows that more than five subjects clearly felt the vibration at \#14, \#21, and \#13, near the hosing or coupling.
The hard contact part probably highlighted the vibration perception.

%%%% 皮膚上での出力と周波数比較
\subsubsection*{\textbf{Vibration propagation on skin}}
To analyze the vibration transmission on the skin in detail, we extracted measurement points on the skin from the results of the T-shirt neck-side area and arranged by power and frequency as shown in Fig. \ref{fig:result_ampfreq_comparison}.
\begin{figure}[h]
\begin{center}
\includegraphics[width = 8cm]{figures/result_ampfreq_comparison.png}
\end{center}
\caption{
Result of the vibration transmission conducted on the six subjects' skin in the neck-side area.
}
\label{fig:result_ampfreq_comparison}
\end{figure}
Table \ref{tab:dampingRate} lists the damping percent, calculated from $ACC_{RMS}$ of \#7 divided by that of \#8 times one hundred.
\begin{table}[]
\centering
\caption{
The damping percent between \#7 and \#8
}
\label{tab:dampingRate}
\scalebox{1}
{
\begin{tabular}{r|ccccccc}
Signal type & sub-1 & sub-2 & sub-3 & sub-4 & sub-5 & sub-6 & AVG. \\ \hline
20Hz-0.5W & 38.0 & 44.9 & 73.1 & 29.6 & 42.6 & 50.2 & 46.4 \\
20Hz-1W & 38.1 & 37.4 & 51.1 & 31.8 & 37.9 & 48.7 & 40.8 \\
20Hz-2W & 38.0 & 36.4 & 42.5 & 32.1 & 36.0 & 45.7 & 38.5 \\
\hline
20Hz-1W & 38.1 & 37.4 & 51.1 & 31.8 & 37.9 & 48.7 & 40.8  \\
80Hz-1W & 49.2 & 30.5 & 25.5 & 26.2 & 16.8 & 11.0 & 26.5 \\
140Hz-1W & 17.5 & 21.8 & 12.0 & 14.6 & 8.4  & 7.3  & 13.6
\end{tabular}
}
\end{table}

%% 定量
% 出力が大きくなっても遠方点ではあまり大きくならない?
For the comparison of the output (Fig. \ref{fig:result_ampfreq_comparison} left column), the transmitted vibration increased for all subjects as the output increased.
The damping tended to intense as the output increased except for sub-1 and sub-4.
"For the comparison of the frequency (Fig. \ref{fig:result_ampfreq_comparison} right column), the overall transmitted vibration decreased as the frequency increased.
The damping tended to be intense as the frequency increased for all subjects."

%% 主観
%出力比較では目立った差はなかったが、周波数比較では明確に高周波数ほど感じにくくなっていた。
The subjective results show little difference between outputs, whereas the perceived intensity decreased as the frequency increased.
"Notably, at \#3 and \#13, only one subject clearly felt the 80 Hz vibration, whereas four subjects clearly felt the 20-Hz vibration, which is similar $ACC_{RMS}$ as that of 80Hz-1W.
Additionally, most subjects could felt no sensation of 80-Hz and 140-Hz vibration at the distant points (\#6 and \#7)."

% FFTした結果
\subsubsection*{\textbf{Fourier transform}}
To verify the fidelity of the transmitted vibration to the skin, we obtained the frequency component from the obtained data via Fast Fourier Transform (FFT).
The data of three axes were converted to one axis by principal component analysis.

"The waveform and FFT results of 20Hz-1W at \#8 in the neck-side area and \#6 in the nape area are shown in Fig. \ref{fig:result_fft}. 
As a representative, we selected data that included a high percentage of high frequency (sub-2 for the neck-side and sub-1 for the nape) and 20 Hz (sub-6 for both areas)."

\begin{figure}[hbt]
\begin{center}
\includegraphics[width = 8cm]{figures/fft_result.png}
\end{center}
\caption{
Waveform of principal axis and result of Fourier transform.
The top graph in the each corners shows principal axis of acceleration signal from 20 Hz sine wave input.
The bottom graph shows the result of single-sided amplitude spectrum of acceleration signal.
}
\label{fig:result_fft}
\end{figure}

The vibration transmitted to the subjects with relatively high body-fat-percentage (e.g., sub-6) tended to consist of 20-Hz vibration mainly, and relatively low body-fat-percentages (e.g., sub-1 and sub-2) tended to consist of harmonic vibrations mainly.
The difference in frequency composition of the transmitted vibration on the skin implies that the vibration perception probably differs depending on the subject's body type, body composition, or worn condition.

%% マネキンで再現可能な周波数応答の測定。目的：20Hz未満の低周波を含む、広範囲の周波数応答を再現可能な手法で測定する。
\subsection{Frequency response of the Hapbeat including below 20 Hz}
\label{exp:freqResponse}
To determine whether the Hapbeat can output low-frequency vibrations below 20 Hz, we measured the frequency response of the Hapbeat with a reproducible method.
"A mannequin, made from a public 3D model and by a 3D-printer, was used as a reproducible wearer (Fig. \ref{fig:desc_mannequin}).
A commercial gel sheet was used as a substitute for human skin."
The details are shown below.
Mannequin 3d data: "haf020.obj" from AIST/HQL Human Body Size and Shape Database 2003 \cite{AIST/HQL2003}.
Making method: The model was divided into sections as shown in Fig. \ref{fig:desc_mannequin} (a), (b), and each section was 3D-printed (material: Z-PLA Pro, laminate thickness: 0.29 mm, infill: 10\% hexagonal). The printed parts were attached with double-sided tape.
Gel sheet: The gel sheet (H0-3K, EXSEAL) is sticky on one side, and the other is smooth, covered with a urethane film.
"The sheet is cut into 50 $\times$ 500 mm and attached to around the neck part of the mannequin.
The other sheet is cut into 230 $\times$ 290 mm and attached to the chest part of the mannequin."
The experimental environment is shown in Fig. \ref{fig:desc_mannequin} (c)--(e).
Measurements were taken at four locations: on the housing, front (Fig. \ref{fig:desc_mannequin} (c)), side(Fig. \ref{fig:desc_mannequin} (d)), and back (Fig. \ref{fig:desc_mannequin} (e)).
The accelerometer was directly applied on the Hapbeat housing or ribbon by the double-sided tape.
The same measurement was also performed with the Vp2 to compare the frequency response of the linear vibrator and that of Hapbeat.
The Vp2 was attached to the gel sheet fixed on a flat aluminum plate, and the accelometer was directly applied on the Vp2.
For the input signal, we used 1--270-Hz sine waves, considering the accelerometer's maximum bandwidth response (300 Hz), based on the E12 series described in section \ref{exp:evaluateCircuit}.
The input amplitude of each frequency was adjusted to consume 1 W with the Hapbeat or Vp2.

% マネキン関連説明
\begin{figure}[hbt]
\begin{center}
\includegraphics[width = 8cm]{figures/desc_mannequin.png}
\end{center}
\caption{
"Division drawing of the mannequin to 3D-print (a)--(b) and measurement conditions (c)--(e).
The texts in (a) indicate the dimensions: $a$ = 150 mm, $b$ = 62.5 mm, $c$ = 1100 mm, $d$ = 70 mm."
The texts in (a) indicate the dimensions: $a$ = 150 mm, $b$ = 62.5 mm, $c$ = 1100 mm, $d$ = 70 mm.
The red and blue lines in (a) correspond to those in (b).
The green arrows in (c)--(e) indicate the direction of the x-axis of the accelerometer.
}
\label{fig:desc_mannequin}
\end{figure}

\subsubsection*{\textbf{Result \& Discussion}}
\begin{figure}[hbt]
\begin{center}
\includegraphics[width = 8cm]{figures/mannequin_result.png}
\end{center}
\caption{
Result of the frequency response of Hapbeat and Vp2 using the mannequin.
The blue horizontal line shows the amplitude of 10 $/mathrm{m/s^2}$.
}
\label{fig:mannequin_result}
\end{figure}

"The result shown in Fig. \ref{fig:mannequin_result} demonstrate $ACC_{RMS}$ exceeded 10 $\mathrm{m \cdot s^{-2}}$ at 3.3 Hz for the housing, 4.7 Hz for the front, and 5.6 Hz for the side.
"
This demonstrates that Hapbeat can generate powerful vibration from input signals below 10 Hz.
The Vp2 cannot output over 1 $\mathrm{m \cdot s^{-2}}$ below 20 Hz, demonstrating unsuitable for vibrating low-frequency range.

% % 目的：筐体への組み込みによる影響が、触覚刺激の知覚に影響するどうかを検証する。胴巻き型との比較
\subsection*{Experiment 2: Comparing the Hapbeat and DC motor}

% 消費電力と発熱について比較。目的：DCを使用しない場合にどれだけ消費電力や発熱量が減るかを調べるため。
\subsection{Comparing the power consumption and heat generation}
\label{exp:powerConsumption}
We derived the power consumption with and without direct current (DC) applied to verify the contribution of the steady-state torque generated by the rubber cord to power saving. 
% DC測定の手順
The measurement with DC (named DC case) and determined as follows.
The Hapbeat includes two motors, and its weight is 58.5 grams plus connected cable mass. Thus, the tension applied on each motor will be about 0.3 N for regular usage.
"With three rounds of thread wound on a bobbin, the thread was attached to a digital force gauge (FPG-5, Nidec-Shimpo Corporation), and it measured the tension.
A power supply (PW18-1.8Q, Kenwood TMI Corp.) applied voltage at which the motor generated 0.3 N of tension, and we recorded the current then."
% AC測定の手順
"The measurement without DC (named AC case) was conducted to derive the power consumption of regular usage.
The sub-6 wore the Hapbeat, and the current values were measured three times when the sine waves of 20Hz-1W, 80Hz-1W, and 140Hz-1W were input."
The power consumptions were calculated using $P=RI^{2}$ with the measurement values and the motor resistance of 1.1 $\Omega$.

\subsubsection*{\textbf{Result \& Discussion}}
In the DC case, the motor flowed 0.32 A.
In the AC case, the RMS current value, derived from the average of three measurements, was 0.65 A at 20 Hz, 0.92 A at 80 Hz, and 0.94 A at 140 Hz.
"The results demonstrate that applying the DC increases power consumption by 1.8--2.3 times compared without DC in driving the signal consumed 1 W.
This will increase heat generation and decrease in continuous running time."

% 起動電流の際について検証・目的：起動電圧の値の違いが、触覚刺激の体験に影響を生じるかを検証。
\subsection{Comparing the starting current}
\label{exp:startingCurrent}
This experiment compared the starting current of the Hapbeat and DC motor to investigate the friction effect of the rubber cord and the Teflon tube.
A starting current is defined as a current value when the shaft rotates from a rest state in the DC motor case.
In the Hapbeat case, the starting current is defined as the current value when the thread first moves from rest.
"The Hapbeat was suspended from a hook, with the accelerometer attached to the coupling with the double-sided tape.
The accelerometer was used to detect the first move; its output was displayed on the oscilloscope."

\subsubsection*{\textbf{Result \& Discussion}}
The result of 10 measurements shows the starting currents of the DC motor were all 0.01 A and that of the Hapbeat averaged 0.55 A (the standard deviation was 0.02 A).
% % DC無しの電流実効値の結果から、これが影響あるかを論じる。
The voltage applied at the first move was 0.61 V in the Hapbeat case, indicating that a weak signal below 0.61 V cannot drive the Hapbeat from rest.
Note that the voltage amplitude applied to the motor at 20Hz-0.5W was 1.05 V.

% % 筐体の重さを変化させた場合の、身体に伝わる振動について測定：（今回の組み込みが質量的に最小構成という前提で）適切な筐体質量を検討するため。
\subsection{Effect of the housing mass}
\label{exp:massEffect}
"The steady-state tension of the Hapbeat, a necklace-type, depends on the housing mass which moves during the drive.
This is a big difference from the WTV, a body-wrapped type, and may affect the vibration transmission."
To examine the mass effect, we measured the transmitted vibration with weights attached to the housing.
Seal-type iron weights (19 mm wide, 12 mm long, and 3.5 mm thick) weighing 5 grams each were attached in units of four, and the measurements were taken three times for each total weight masses of 0, 20, 40, 60, 80, 100, and 120 grams.
The fifth and subsequent sheets were pasted on top of the attached weights.
The input signals were 20Hz-0.5W, 20Hz-1W, 20Hz-2W, 80Hz-1W, and 140Hz-1W.
The measurement points were at the \#8 (the neck-side area) and \#6 (the nape area) of the sub-6 wearing the underwear and T-shirt used in the experiment \ref{exp:repeat_exp}.

\subsubsection*{\textbf{Result \& Discussion}}
The neck-side result shown in Fig. \ref{fig:result_mass} demonstrate that $ACC_{RMS}$ of 80 g in the housing mass was the largest at all input signals, and $ACC_{RMS}$ tended to decrease with increasing housing mass at 20-Hz signals.
Although $ACC_{RMS}$ of 80-Hz and 140-Hz input decreases at 100 grams, they do not decrease monotonically.
The nape result seemed a similar trend as the neck-side, to a lesser extent.
\begin{figure}[hbt]
\begin{center}
\includegraphics[width = 8cm]{figures/result_mass.png}
\end{center}
\caption{
Vibration transmission result with the varying housing mass.
}
\label{fig:result_mass}
\end{figure}

% 応答速度の測定
\subsection{Response time of the Hapbeat}
\label{exp:responseTime}
The response speed of the Hapbeat was measured to examine whether the internal friction of the Hapbeat adversely affects the response speed or not.
The Hapbeat hung on a hook-shaped part formed by the 3D-printer and was attached to the sensor tip.
The step voltage was applied by turning on a battery box that contained two 1.2-V AA batteries in series.
"To normalize the measured data, the values before the step voltages were set to zero, and the average value of steady-state after the input was set to one. 
The steady-state was defined as the voltage drifting is within 0.1 V per second.
The time of interest was when the normalized value of the input voltage and tension increased from 0.1 and 0.9."
\subsubsection*{\textbf{Result \& Discussion}}
The average of ten trials was 2.74 ms, and the max value was 3.00 ms.
A previous study \cite{yem2016vibrotactile} has shown that the response time of a coreless DC motor is 3 ms, and thus the result shows the internal friction can be dismissed for the response speed.


==> Don't use/sub6-discussion.tex <==
\section{General discussion}
The present study demonstrate that the proposed necklace-type device, Hapbeat, transmits low-frequency vibrations over a wider area of the user's body.
However, the transmitted vibrations contained a high percentage of harmonic components, even more than the component of inputted low-frequency for some subjects.

"The subjective results demonstrate that most subjects clearly felt 20Hz-1W vibration at multiple locations in all the chest, neck-side, and nape area, especially near the ribbon or housing. 
This also indicates that the Hapbeat transmitted low-frequency vibration perceptually to a wider area."
"The Hapbeat's response speed was 2.74 $\mathbf{m \cdot s^{-2}}$, which is comparable to that of coreless motors or linear vibrators \cite{yem2016vibrotactile}.
The Hapbeat also can outputs high-frequency vibrations, exceeding 10$\mathbf{m \cdot s^{-2}}$ up to 270 Hz, and the vibrations of 80 and 140 Hz were perceivable near the ribbon or housing."
Our findings suggest that the Hapbeat is useful as a wearable vibroacoustic device because it covers a frequency range of 5--270 Hz, a low-frequency range in music, and can respond to impact sounds such as drums or explosions sound with a slight delay.

%%% 先行研究からのメリット
We also succeeded in redesigning WTV as a necklace-type device to improve usability, developing a drive circuit that can draw a high current with audio signals and a battery, and saving power consumption using a rubber cord to generate a steady-state torque.
This achieves the Hapbeat is easy to wear (takes less than five seconds) and can be used anywhere, whereas WTV requires a power source to drive, a structure to fix, and a long time (more than ten seconds) to wear.

We will describe some interesting findings from the experiments in the following subsections.
%% 服の比較
\subsection{Effect of clothings}
Comparing the transmitted vibrations to the T-shirt and dress shirt from Fig. \ref{fig:result_trans_subject}, the dress shirt more effectively transmitted the vibrations to a wider area in both quantitative and subjective results.
This may be due to the higher Young's modulus of the dress shirt fabric.
The $ACC_{RMS}$ of the housing (\#22) was also larger for the dress shirt, suggesting that the T-shirt easily deformed and prevented the housing movement due to its softness.
These results indicate that clothes will affect the vibration transmission from Hapbeat, and a higher Young's modulus clothes may transmit effectively.
This phenomenon may occur with other general vibrators attached to clothes.

\subsection{Vibration propagation by skin surface waves}
The result of the T-shirt neck-side in Fig. \ref{fig:result_ampfreq_comparison} shows the $ACC_{RMS}$ at \#6, 7-cm away from the ribbon, greatly attenuated than that of \#8, near the ribbon.
The vibration transmission of internal skin from the vibrating source to a distant point is known to occur by shear waves, which are primarily through soft tissue in the frequency range of the tactile perception \cite{moore1970survey}.
Dandu et al. \cite{dandu2019spatiotemporal} performed a Fourier expansion of the polarization for an arbitrary plane and presented the equation below for the skin strain vector from the following findings: the equation of motion for elastic bodies, the damping rate and transport rate of viscoelastic skin and soft tissue dependent on the vibration frequency \cite{manfredi2012effect} \cite{pereira1991dynamic}; the solution of strain vectors for time and distance from a vibrating source in soft tissue in a linear viscoelastic model.
\begin{equation*}
\xi ( x,t) =\int ^{\infty }_{-\infty } df\ \phi ( f) \ e^{-axf} \ e^{j2\pi f( x/c( f) \ -\ t)}
\label{eq:kai}
\end{equation*}
where $\xi(x,t)$ is the time-varying strain vector, $x$ is the distance from the vibrating source, $t$ is the time, $f$ is the frequency, and $c(f)$ is the propagation velocity.
In the linear viscoelastic model, the damping is considered to increase almost linearly with frequency, so the damping rate is assumed to be $\sigma = \alpha f$ (where $\alpha$ is an arbitrary constant).
From this, it can be seen that the vibrations decay exponentially with increasing distance and frequency.

"This phenomenon aligns with the results obtained in the experiment; the 
higher input frequency occurs lower damping percent shown in Table \ref{tab:dampingRate}, indicating the skin's viscosity damped the vibration."
The subjective result of Fig. \ref{fig:result_ampfreq_comparison}, the subjects only felt vibration near the ribbon, also support this.

The damping percent slightly decreases as the output increases, but the subjective results are almost the same.
The reason can be that the transmitted vibration of 20Hz-0.5W was well perceptible, and the increased values of $ACC_{RMS}$ at distant locations were relatively small than that at the near ribbon.
Additionally, in all cases, the subjects hardly felt the vibrations at \#6, where 7-cm distant from the ribbon.

"These findings indicate that expanding the contact area of the vibrating part more achieves extensive transmission than increasing the vibration output.
This supports the proposed method, which is a ribbon contacted widely to a user's body actuate the skin, is suitable for the extensive transmission."

%% デメリット。立ち位置的にLimitationか。
\section{Limitation}
The outputs of the low-frequency vibration contained a high percentage of harmonics, which resulted in poor reproducibility of the input signal (Fig. \ref{fig:result_fft}).
Because the Hapbeat is suspended, it cannot actuate the user's skin when it unwinds and loosens the thread.
Thus, the Hapbeat discards the negative voltage part of input signals if we define the positive voltage as it drives the motor to wind the thread.
"The internal friction, derived from the contact between the thread or rubber cord and the Teflon tubes, stops the thread movement occurred by a weak input voltage.
This leads to a rapid and intense actuation when the input voltage exceeds a certain value."
These phenomena may have caused the spike waveform of the vibrations transmitted from the Hapbeat, as shown in Fig. \ref{fig:result_fft}, resulting in a high percentage of harmonics.

The result of the experiment \ref{exp:massEffect} shows the housing mass affects the vibration transmission.
"This implies that changing the steady-state tension could control the transmission characteristics, e.g., emphasizing high-frequency vibrations or vibrations transmitted to the nape area.
However, the steady-state tension of the Hapbeat is difficult to control because it depends on the housing mass."
The 20-Hz vibrations decreased when the housing mass exceeded 80 grams.
"The larger steady-state tension, caused by heavier housing mass, maximally stretches the rubber cord, limiting the maximum angular displacement of the bobbin.
This limitation possibly causes the decrement, considering actuating low-frequency vibrations requires a longer stroke of actuators. "
Increasing the rubber cord length can solve this problem, but it will cause other problems such as increasing the housing volume or internal friction.

% 実験手法のLimitation
The subjects of the experiments were only six males, and transmitted vibrations at some measurement points showed quite large individual differences.
Thus, additional experiments considering more conditions such as subjects' body type and the contact state of the ribbon to derive a general vibration transfer function of Hapbeat.

% 振動伝達だけ考えれば巻き付け＆DCによる定常張力の方が好ましい
"These negative results indicate that Hapbeat is an unsuitable device for transmitting vibration fidelity to an input signal.
The following modifications, which improve the usability, will increase the number of factors that affect the transmission: using a rubber cord to generate steady-state tension, incorporating the mechanism into the housing, and wearing a device like a necklace."
% 体感音響ではエンベロープが周波数より重要(?)
However, the main usage of Hapbeat is the vibroacoustic effect.
"Auditory researches have showed that a brain tracks the envelope of speech and music \cite{di2020cortical}\cite{cantisani2019eeg}.
This fact may imply a device used for the vibroacoustic effect is required envelope fidelity rather than frequency fidelity.
% そもそも服による（悪？）影響の方がWTV➡Hapbeatになる影響よりも大きいのでは
In actual use-case, the effects of clothing type will have an impact on the transmission.
Thus, additional experiments are required to determine the extent to which the disadvantages will affect the perception of the vibroacoustic effect.


==> Don't use/sub7-conclusion.tex <==
\section{Conclusion}
This paper proposed a necklace-type haptic device, Hapbeat, and the experimental results demonstrated that it could transmit high-power, low-frequency vibrations over a wider area.
The results also show the response speed is comparable to linear vibrators, and the Hapbeat can output well perceptible vibration by 5--270-Hz sine wave input.
Thus, our proposed method enables developing a small vibroacoustic device that can transmit the powerful low-frequency vibration over a wider area, which is difficult to achieve with conventional devices.
Although this paper focused on the necklace-type, this method can be applied to various wearable haptic devices such as belt-type or wristband-type. 
The vibroacoustic effect is a special experience that can only be experienced in certain facilities or limited environments.
We hope our proposal makes enjoying the vibroacoustic effect less special and creates new ways of using vibroacoustic effects. 

